Combining chains of Bayesian models with Markov melding

A challenge for practitioners of Bayesian inference is specifying a model that incorporates multiple relevant, heterogeneous data sets. It may be easier to instead specify distinct submodels for each source of data, then join the submodels together. We consider chains of submodels, where submodels directly relate to their neighbours via common quantities which may be parameters or deterministic functions thereof. We propose chained Markov melding, an extension of Markov melding, a generic method to combine chains of submodels into a joint model. One challenge we address is appropriately capturing the prior dependence between common quantities within a submodel, whilst also reconciling differences in priors for the same common quantity between two adjacent submodels. Estimating the posterior of the resulting overall joint model is also challenging, so we describe a sampler that uses the chain structure to incorporate information contained in the submodels in multiple stages, possibly in parallel. We demonstrate our methodology using two examples. The first example considers an ecological integrated population model, where multiple data sets are required to accurately estimate population immigration and reproduction rates. We also consider a joint longitudinal and time-to-event model with uncertain, submodel-derived event times. Chained Markov melding is a conceptually appealing approach to integrating submodels in these settings.

==> tex-input/arbitrary-graphs/0010-example-model-graph.tex <==
\begin{figure}[tb]
  \centering
  \begin{tikzpicture}[> = stealth, node distance = 1.5cm, thick, state/.style={draw = none, minimum width = 1.25cm}]
  % nodes 
  \node [state] (model-1) {$\pd_{1}$};
  \node [state] [above left = of model-1](model-2) {$\pd_{2}$};
  \node [state] [above right = of model-1](model-3) {$\pd_{3}$};
  \node [state] [right = of model-3](model-4) {$\pd_{4}$};
  \node [state] [below  = of model-1](model-5) {$\pd_{5}$};

  % edges
  \path[->] (model-2) edge node[above right] {$\phi_{1 \cap 2}$} (model-1);
  \path[->] (model-4) edge node[above] {$\phi_{3 \cap 4}$} (model-3);

  \path (model-3) edge node[above left] {$\phi_{1 \cap 3}$} (model-1);
  \path (model-1) edge node[right] {$\phi_{1 \cap 5}$} (model-5);

  \end{tikzpicture}
  \caption{An arbitrary graph connected by common quantities $\phi_{\modelindex \cap \modelindex'}$.}
  \label{fig:example-model-graph}
\end{figure}

==> tex-input/arbitrary-graphs/0011-example-model-graph.tex <==
\begin{figure}[tb]
  \centering
  \begin{tikzpicture}[> = stealth, node distance = 1.5cm, thick, state/.style={draw = none, minimum width = 1.25cm}]
  % nodes 
  \node [state] (model-1) {$\pd_{1}$};
  \node [state] [above right = of model-1] (model-3) {$\pd_{3}$};
  \node [state] [above = of model-3] (model-4) {$\pd_{4}$};
  \node [state] [below = of model-1] (model-5) {$\pd_{5}$};

  \coordinate [above left of = model-1] (blank2);

  \node [state] [above = 2.3cm of blank2] (model-2) {$\pd_{2}$};

  % edges
  \path[->] (model-2) edge[out = 270, in = 135] node [above right] (phi-12) {$\phi_{1 \cap 2}$} (model-1);
  \path[->] (model-4) edge node [right] (phi-34) {$\phi_{3 \cap 4}$} (model-3);

  \path (model-3) edge node [below right] (phi-13) {$\phi_{1 \cap 3}$} (model-1);
  \path (model-1) edge node [right] (phi-15) {$\phi_{1 \cap 5}$} (model-5);

  % stage one - blue
  \node (stage-1) [draw = mymidblue, fit = (model-4) (phi-34), inner sep = 0.05cm, dotted] {};
  \node (stage-1-label) [yshift = 1.5ex, mymidblue] at (stage-1.north east) {$s_{1}$};
  \node (stage-1-prime) [draw = mymidblue, fit = (model-2) (phi-12), inner sep = 0.05cm, dotted] {};
  \node (stage-1-prime-label) [yshift = 1.5ex, mymidblue] at (stage-1-prime.north east) {$s_{1}'$};

  % stage two - grey
  \node (stage-2) [draw = mydarkblue, fit = (model-3) (model-4) (phi-13) (phi-34) (stage-1-label), inner sep = 0.1cm, dotted] {};
  \node (stage-2-label) [yshift = 1.5ex, mydarkblue] at (stage-2.north east) {$s_{2}$};

  % stage three - red
  \node (stage-3) [draw = myredhighlight, fit = (model-1) (model-2) (model-4) (phi-15) (phi-34) (stage-2-label), inner sep = 0.135cm, dotted] {};
  \node (stage-3-label) [yshift = 1.5ex, myredhighlight] at (stage-3.north east) {$s_{3}$};

  % stage four - black
  \node (stage-4) [draw = black, fit = (model-2) (model-4) (model-5) (phi-34) (stage-3-label), inner sep = 0.225cm] {};
  \node [yshift = 1.5ex, black] at (stage-4.north east) {$s_{4}$};

  \end{tikzpicture}
  \caption{An arbitrary graph connected by common quantities $\phi_{\modelindex \cap \modelindex'}$. The bounding boxes represent the models considered in stage $s_{\modelindex}$ of the multi-stage sampler.}
  \label{fig:example-model-graph-top-down}
\end{figure}

==> tex-input/dc-sampler/0000-tikz-target.tex <==
\begin{figure}[tb]
  \centering
  \begin{tikzpicture}[node distance = 1.5cm, thick, state/.style={draw = none, minimum width = 1.25cm}]  
  % Nodes
  \node [state] (model-1) {$\textcolor{mymidblue}{\pd_{1}}$};
  \node [state] [above right = of model-1] (model-2) {$\textcolor{mymidblue}{\pd_{2}}$};
 
  \coordinate [right of = model-2] (blank1);

  \node [state] [right of = blank1] (model-Kminus1) {$\textcolor{mymidblue}{\pd_{k - 1}}$};
  \node [state] [below right = of model-Kminus1] (model-K) {$\pd_{k}$};
  \node [state] [above right = of model-K] (model-Kplus1) {$\textcolor{myredhighlight}{\pd_{k + 1}}$};

  \coordinate [right of = model-Kplus1] (blank2);
  
  \node [state] [right = of blank2] (model-Mminus1) {$\textcolor{myredhighlight}{\pd_{\Nm - 1}}$};
  \node [state] [below right = of model-Mminus1] (model-M) {$\textcolor{myredhighlight}{\pd_{\Nm}}$};

  \coordinate [below of = model-1] (blank3);
  \coordinate [below of = model-K] (blank4);
  \coordinate [below of = model-M] (blank5);
  

  % Edges
  \draw (model-1) edge node[above left] {$\textcolor{mymidblue}{\phi_{1 \cap 2}}$} (model-2);

  \draw [dotted] (model-2) edge (model-Kminus1);

  \draw (model-Kminus1) edge node[above right] {$\textcolor{mymidblue}{\phi_{k - 1 \cap k}}$} (model-K);
  \draw (model-K) edge node[above left] {$\textcolor{myredhighlight}{\phi_{k \cap k + 1}}$} (model-Kplus1);

  \draw [dotted] (model-Kplus1) edge (model-Mminus1);

  \draw (model-Mminus1) edge node[above right] {$\textcolor{myredhighlight}{\phi_{\Nm - 1 \cap \Nm}}$} (model-M);

  % \draw [<->](model-1.south) -- (model-K.south);

  \end{tikzpicture}
  \caption{Divide and conquer sampler overview}
  \label{fig:dc-tikz-target}
\end{figure}

==> tex-input/dc-sampler/0010-dc-final-target.tex <==
\begin{multline}
  \pd_{\text{meld}}(\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{1}, \ldots, \psi_{\Nm} \mid Y_{1}, \ldots, Y_{\Nm}) \propto \\ 
  \frac {
      \pd_{1} (\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
  \prod_{\modelindex = 2}^{\Nm - 1} \left\{
    \frac {
      \pd_{\modelindex} (\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1}, \psi_{\modelindex}, Y_{\modelindex})
    } {
      \pd_{\modelindex}(\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1})
    }
  \right\}
  \frac {
    \pd_{\Nm} (\phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm}, Y_{\Nm})
  } {
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm})
  }
  \pd_{\text{pool}}(\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}) 
  \label{eqn:dc-final-target}
\end{multline}

==> tex-input/dc-sampler/0011-dc-gibbs-updates.tex <==
\begin{align}
  \textcolor{mymidblue}{
    \phi_{1 \cap 2}, \ldots, \phi_{k - 1 \cap k},
    \psi_{1}, \ldots, \psi_{k - 1}
  }
    \mid
    \phi_{k + 1 \cap k} \ldots, \phi_{\Nm - 1 \cap \Nm},
    \psi_{k},
    \psi_{k + 1}, \ldots, \psi_{\Nm} 
  \,\, &\sim \,\, 
    \textcolor{mymidblue}{
      \pd_{\text{meld}, \textcolor{mymidblue}{A}}
    }
   \\
  \textcolor{myredhighlight}{
    \phi_{k \cap k + 1} \ldots, \phi_{\Nm - 1 \cap \Nm},
    \psi_{k + 1}, \ldots, \psi_{\Nm}
  }
    \mid
    \phi_{1 \cap 2}, \ldots, \phi_{k - 1 \cap k},
    \psi_{1}, \ldots, \psi_{k - 1},
    \psi_{k}
   \,\, &\sim \,\, 
    \textcolor{myredhighlight}{
      \pd_{\text{meld}, \textcolor{myredhighlight}{B}}
    }
   \\
  \psi_{k} 
  \mid 
  \phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm},
  \psi_{1}, \ldots, \psi_{k-1}, \psi_{k + 1}, \ldots, \psi_{\Nm} 
  \,\, &\sim \,\, 
  \q(\psi_{k}^{*} \mid \psi_{k})
  \label{eqn:dc-gibbs-updates}
\end{align}

==> tex-input/dc-sampler/0012-dc-acceptance-probabilities.tex <==
\begin{multline}
  \alpha \left(
    (\phi_{1 \cap 2}^{*}, \ldots, \phi_{k - 1 \cap k}^{*}, \psi_{1}^{*}, \ldots, \psi_{k - 1}^{*}),
    (\phi_{1 \cap 2}, \ldots, \phi_{k - 1 \cap k}, \psi_{1}, \ldots, \psi_{k - 1})
  \right)
  =\\ 
  \frac {
    \pd_{k}(\phi_{k - 1 \cap k}^{*}, \phi_{k \cap k + 1}, \psi_{k}, Y_{k})
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1})
    \pd_{\text{pool}}(\phi_{1 \cap 2}^{*}, \ldots, \phi_{k - 1 \cap k}^{*}, \phi_{k \cap k + 1}, \ldots, \phi_{\Nm - 1})
  } {
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1}, \psi_{k}, Y_{k})
    \pd_{k}(\phi_{k - 1 \cap k}^{*}, \phi_{k \cap k + 1})
    \pd_{\text{pool}}(\phi_{1 \cap 2}, \ldots, \phi_{k - 1 \cap k}, \phi_{k \cap k + 1}, \ldots, \phi_{\Nm - 1})
  }
  \end{multline}
  \begin{multline}
  \alpha \left(
    (\phi_{k \cap k + 1}^{*} \ldots, \phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{k + 1}^{*}, \ldots, \psi_{\Nm}^{*}),
    (\phi_{k \cap k + 1} \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{k + 1}, \ldots, \psi_{\Nm})
  \right)
  =\\
  \frac {
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1}^{*}, \psi_{k}, Y_{k})
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1})
    \pd_{\text{pool}}(\phi_{1 \cap 2}, \ldots, \phi_{k - 1 \cap k}, \phi_{k \cap k + 1}^{*}, \ldots, \phi_{\Nm - 1}^{*})
  } {
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1}, \psi_{k}, Y_{k})
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1}^{*})
    \pd_{\text{pool}}(\phi_{1 \cap 2}, \ldots, \phi_{k - 1 \cap k}, \phi_{k \cap k + 1}, \ldots, \phi_{\Nm - 1})
  } 
  \end{multline}
  \begin{equation}
  \alpha \left(
    (\psi_{k}^{*}),
    (\psi_{k})
  \right)
  = 
  \frac {
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1}, \psi_{k}^{*}, Y_{k})
    \q(\psi_{k} \mid \psi_{k}^{*})
  } {
    \pd_{k}(\phi_{k - 1 \cap k}, \phi_{k \cap k + 1}, \psi_{k}, Y_{k})
    \q(\psi_{k}^{*} \mid \psi_{k})
  }
  \label{eqn:dc-acceptance-probabilities}
\end{equation}

==> tex-input/dc-sampler/0022-stage-one-acceptance-probs.tex <==
\begin{align}
  \alpha((\phi_{1 \cap 2}^{*}, \psi_{1}^{*}), (\phi_{1 \cap 2}, \psi_{1})) &= 
  \frac {
    \pd_{\text{pool}, 1} (\phi_{1 \cap 2}^{*})
  } {
    \pd_{\text{pool}, 1} (\phi_{1 \cap 2})
  }
  \frac {
    \pd_{1}(\phi_{1 \cap 2}^{*}, \psi_{1}^{*}, Y_{1})
    \pd_{1}(\phi_{1 \cap 2})
  } {
    \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    \pd_{1}(\phi_{1 \cap 2}^{*})
  }
  \frac {
    \q(\phi_{1 \cap 2}, \psi_{1} \mid \phi_{1 \cap 2}^{*}, \psi_{1}^{*})
  } {
    \q(\phi_{1 \cap 2}^{*}, \psi_{1}^{*} \mid \phi_{1 \cap 2}, \psi_{1})
  } \\
  \alpha((\phi_{2 \cap 3}^{*}, \psi_{3}^{*}), (\phi_{2 \cap 3}, \psi_{3})) &= 
  \frac {
    \pd_{\text{pool}, 3} (\phi_{2 \cap 3}^{*})
  } {
    \pd_{\text{pool}, 3} (\phi_{2 \cap 3})
  }
  \frac {
    \pd_{3}(\phi_{2 \cap 3}^{*}, \psi_{3}^{*}, Y_{3})
    \pd_{3}(\phi_{2 \cap 3})
  } {
    \pd_{3}(\phi_{2 \cap 3}, \psi_{3}, Y_{3})
    \pd_{3}(\phi_{2 \cap 3}^{*})
  }
  \frac {
    \q(\phi_{2 \cap 3}, \psi_{3} \mid \phi_{2 \cap 3}^{*}, \psi_{3}^{*})
    } {
    \q(\phi_{2 \cap 3}^{*}, \psi_{3}^{*} \mid \phi_{2 \cap 3}, \psi_{3})
  },  
  \label{eqn:stage-one-acceptance-probs}  
\end{align}

==> tex-input/dc-sampler/0023-stage-one-acceptance-probs.tex <==
\begin{align}
  \alpha((\phi_{1 \cap 2}^{*}, \psi_{1}^{*}), (\phi_{1 \cap 2}, \psi_{1})) &= 
  \frac {
    \pd_{1}(\phi_{1 \cap 2}^{*}, \psi_{1}^{*}, Y_{1})
    \pd_{1}(\phi_{1 \cap 2})
  } {
    \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    \pd_{1}(\phi_{1 \cap 2}^{*})
  }
  \frac {
    \q(\phi_{1 \cap 2}^{*}, \psi_{1}^{*} \mid \phi_{1 \cap 2}, \psi_{1})
  } {
    \q(\phi_{1 \cap 2}, \psi_{1} \mid \phi_{1 \cap 2}^{*}, \psi_{1}^{*})
  } \\
  \alpha((\phi_{2 \cap 3}^{*}, \psi_{3}^{*}), (\phi_{2 \cap 3}, \psi_{3})) &= 
  \frac {
    \pd_{3}(\phi_{2 \cap 3}^{*}, \psi_{3}^{*}, Y_{3})
    \pd_{3}(\phi_{2 \cap 3})
  } {
    \pd_{3}(\phi_{2 \cap 3}, \psi_{3}, Y_{3})
    \pd_{3}(\phi_{2 \cap 3}^{*})
  }
  \frac {
    \q(\phi_{2 \cap 3}^{*}, \psi_{3}^{*} \mid \phi_{2 \cap 3}, \psi_{3})
  } {
    \q(\phi_{2 \cap 3}, \psi_{3} \mid \phi_{2 \cap 3}^{*}, \psi_{3}^{*})
  }  
  \label{eqn:stage-one-acceptance-probs}  
\end{align}

==> tex-input/introduction/0001-intro-dag.tex <==
\begin{figure}[tb]
  \centering
  \begin{tikzpicture}[> = stealth, node distance = 1.5cm, thick, state/.style={draw = none, minimum width = 1.25cm}]
  % nodes 
  \node [state] (model-1) {$\pd_{1}$};
  \node [state] [right = of model-1](model-2) {$\pd_{2}$};
  \node [state] [right = of model-2](model-3) {$\pd_{3}$};

  % edges
  \path[-] (model-1) edge node[above] {$\phi_{1 \cap 2}$} (model-2);
  \path[-] (model-2) edge node[above] {$\phi_{2 \cap 3}$} (model-3);
  \end{tikzpicture}
  \caption{A DAG of the simplest submodel relationship structure of interest. Nodes represent submodels $\pd_{\modelindex}$, and labelled edges represent quantities common to both submodels $\phi_{\modelindex \cap \modelindex'}$.}
  \label{fig:intro-dag}
\end{figure}

==> tex-input/mimic-example/0011-pf-model-priors-simple.tex <==
\begin{equation}
  \beta_{0, i} \sim \text{N}(0, 1^2), \qquad \varepsilon_{i, j} \sim t_{5}(0, \omega_{i}), \qquad  \omega_{i} \sim \text{N}_{+}(0, 1^2).
  \label{eqn:pf-model-priors-simple}
\end{equation}

==> tex-input/mimic-example/0021-fluid-submodel-noise-priors.tex <==
\begin{equation}
  \epsilon_{i, l} \sim \text{N}(0, \sigma^{2}_{x, i}),  \,\, \sigma_{x, i} \sim \text{N}_{+}(0, 5^2),
\end{equation}

==> tex-input/mimic-example/0022-fluid-submodel-slope-priors.tex <==
\begin{equation}
  \eta^{b}_{1, i} \sim \text{Gamma}(1.53, 0.24), \,\, \eta^{a}_{1, i} \sim \text{Gamma}(1.53, 0.24).
\end{equation}

==> tex-input/multi-stage-sampler/0010-melded-posterior.tex <==
\begin{equation}
  \pd_{\text{meld}} (\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, \psi_{3}, \mid Y_{1}, Y_{2}, Y_{3})
  \propto
  \pd_{\text{meld}} (\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, \psi_{3}, Y_{1}, Y_{2}, Y_{3})
  \label{eqn:melded-posterior}
\end{equation}

==> tex-input/multi-stage-sampler/0040-stage-Mminus1-target.tex <==
\begin{multline}
  \pd_{\text{meld}, \Nm - 1}(\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{1}, \ldots, \psi_{\Nm - 1} \mid Y_{1}, \ldots, Y_{\Nm - 1}) \propto \\
  \frac {
    \pd_{1} (\phi_{1 \cap 2}, \psi_{1}, Y_{1})
  } {
    \pd_{1}(\phi_{1 \cap 2})
  }
  \prod_{\modelindex = 2}^{\Nm - 1} \left\{
    \frac {
      \pd_{\modelindex} (\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1}, \psi_{\modelindex}, Y_{\modelindex})
    } {
      \pd_{\modelindex}(\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1})
    }
  \right\}
  \label{eqn:stage-Mminus1-target}
\end{multline}\\

==> tex-input/multi-stage-sampler/0041-stage-Mminus1-gibbs-updates.tex <==
\begin{align}
  \phi_{1 \cap 2}^{*}, \ldots, \phi_{\Nm - 2 \cap \Nm - 1}^{*}, \psi_{1}^{*}, \ldots, \psi_{\Nm - 1}^{*} \mid \phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm} 
    &\sim 
    \pd_{\text{meld}, \Nm - 2}
  \\
  \phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{\Nm}^{*} \mid \phi_{1 \cap 2}, \ldots, \phi_{\Nm - 2 \cap \Nm - 1}, \psi_{1}, \ldots, \psi_{\Nm - 1} 
    &\sim
    \q(\phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{\Nm}^{*} \mid \phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm})
  \label{eqn:stage-Mminus1-gibbs-updates}
\end{align}

==> tex-input/multi-stage-sampler/0042-stage-Mminus1-acceptance-probabilities.tex <==
\begin{multline}
  \alpha\left(
    (\phi_{1 \cap 2}^{*}, \ldots, \phi_{\Nm - 2 \cap \Nm - 1}^{*}, \psi_{1}^{*}, \ldots, \psi_{\Nm - 2}^{*}),
    (\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 2 \cap \Nm - 1}, \psi_{1}, \ldots, \psi_{\Nm - 2})
  \right)
  = \\
  \frac {
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}^{*}, \phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm - 1}, Y_{\Nm - 1})
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}, \phi_{\Nm - 1 \cap \Nm})
  } {
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}, \phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm - 1}, Y_{\Nm - 1})
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}^{*}, \phi_{\Nm - 1 \cap \Nm})
  } 
  \end{multline}
  \begin{multline}
  \alpha\left(
    (\phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{\Nm - 1}^{*}),
    (\phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm - 1})
  \right)
  = 
  \frac {
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}, \phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{\Nm - 1}^{*}, Y_{\Nm - 1})
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}, \phi_{\Nm - 1 \cap \Nm})
  } {
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}, \phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm - 1}, Y_{\Nm - 1})
    \pd_{\Nm - 1}(\phi_{\Nm - 2 \cap \Nm - 1}, \phi_{\Nm - 1 \cap \Nm}^{*})
  } 
  % \label{eqn:Mminus1-acceptance-probabilities}
\end{multline}

==> tex-input/multi-stage-sampler/0050-stage-M-target.tex <==
\begin{multline}
  \pd_{\text{meld}, \Nm'}(\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{1}, \ldots, \psi_{\Nm} \mid Y_{1}, \ldots, Y_{\Nm}) \propto \\ 
  \frac {
      \pd_{1} (\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
  \prod_{\modelindex = 2}^{\Nm - 1} \left\{
    \frac {
      \pd_{\modelindex} (\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1}, \psi_{\modelindex}, Y_{\modelindex})
    } {
      \pd_{\modelindex}(\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1})
    }
  \right\}
  \frac {
    \pd_{\Nm} (\phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm}, Y_{\Nm})
  } {
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm})
  }
  \label{eqn:stage-M-target}
\end{multline}

==> tex-input/multi-stage-sampler/0051-stage-M-gibbs-updates.tex <==
\begin{align}
  \phi_{1 \cap 2}^{*}, \ldots, \phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{1}^{*}, \ldots, \psi_{\Nm - 1}^{*} \mid \psi_{\Nm} 
    \sim & \, 
    \pd_{\text{meld}, \Nm - 1}
  \\
  \psi_{\Nm}^{*} \mid \phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{1}, \ldots, \psi_{\Nm - 1}
    \sim & \,
    \q(\psi_{\Nm}^{*} \mid \psi_{\Nm})
  \label{eqn:stage-M-gibbs-updates}
\end{align}

==> tex-input/multi-stage-sampler/0052-stage-M-acceptance-probabilities.tex <==
\begin{align}
  \alpha\left(
    (\phi_{1 \cap 2}^{*}, \ldots, \phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{1}^{*}, \ldots, \psi_{\Nm - 1}^{*}),
    (\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{1}, \ldots, \psi_{\Nm - 1})
  \right)
  &= 
  \frac {
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{\Nm}, Y_{\Nm})
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm})
  } {
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm}, Y_{\Nm})
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm}^{*})
  } \\ 
  \alpha\left(
    (\psi_{\Nm}^{*}),
    (\psi_{\Nm})
  \right)
  &=  
  \frac {
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm}^{*}, Y_{1})
  } {
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm}, Y_{1})
  } 
  \label{eqn:stage-M-acceptance-probabilities}
\end{align}

==> tex-input/multi-stage-sampler/0060-stage-Mplus1-target.tex <==
\begin{multline}
  \pd_{\text{meld}}(\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{1}, \ldots, \psi_{\Nm} \mid Y_{1}, \ldots, Y_{\Nm}) \propto \\ 
  \frac {
      \pd_{1} (\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
  \prod_{\modelindex = 2}^{\Nm - 1} \left\{
    \frac {
      \pd_{\modelindex} (\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1}, \psi_{\modelindex}, Y_{\modelindex})
    } {
      \pd_{\modelindex}(\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1})
    }
  \right\}
  \frac {
    \pd_{\Nm} (\phi_{\Nm - 1 \cap \Nm}, \psi_{\Nm}, Y_{\Nm})
  } {
    \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm})
  }
  \pd_{\text{pool}}(\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}) 
  \label{eqn:stage-Mplus1-target}
\end{multline}

==> tex-input/multi-stage-sampler/0061-stage-Mplus1-update.tex <==
\begin{equation}
  \phi_{1 \cap 2}^{*}, \ldots, \phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{1}^{*}, \ldots, \psi_{\Nm}^{*} 
    \sim \, 
    \pd_{\text{meld}, \Nm'}
  \label{eqn:stage-Mplus1-update}
\end{equation}

==> tex-input/multi-stage-sampler/0062-stage-Mplus1-acceptance-probability.tex <==
\begin{equation}
  \alpha \left(
    (\phi_{1 \cap 2}^{*}, \ldots, \phi_{\Nm - 1 \cap \Nm}^{*}, \psi_{1}^{*}, \ldots, \psi_{\Nm}^{*}),
    (\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}, \psi_{1}, \ldots, \psi_{\Nm})
  \right)
  =
  \frac {
    \pd_{\text{pool}}(\phi_{1 \cap 2}^{*}, \ldots, \phi_{\Nm - 1 \cap \Nm}^{*})
  } {
    \pd_{\text{pool}}(\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm})
  }
  \label{eqn:stage-Mplus1-acceptance-probability}
\end{equation}

==> tex-input/multiple-phi/0002-submodel-two-marginal-replacement.tex <==
\begin{equation}
  \pd_{\text{repl}, 2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2}) = 
  \pd_{\text{pool}}(\phi_{1 \cap 2}, \phi_{2 \cap 3})
  \frac {
    \pd_{2} (\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2})
  } {
    \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})
  }.
  \label{eqn:submodel-two-marginal-replacement}
\end{equation}

==> tex-input/multiple-phi/0012-melded-model-full.tex <==
\begin{equation}
  \pd_{\text{pool}}(\phi_{1 \cap 2}, \phi_{2 \cap 3})
  \frac {
    \pd_{1} (\phi_{1 \cap 2}, \psi_{1}, Y_{1})
  } {
    \pd_{1}(\phi_{1 \cap 2})
  }
  \frac {
    \pd_{2} (\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2})
  } {
    \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})
  }
  \frac {
    \pd_{3} (\phi_{2 \cap 3}, \psi_{3}, Y_{3})
  } {
    \pd_{3}(\phi_{2 \cap 3})
  }.
  \label{eqn:melded-model-full}
\end{equation}

==> tex-input/multiple-phi/0020-stage-two-proposals.tex <==
\begin{align}
  \phi_{1}^{*} \mid \phi_{2}, \psi_{1}, \psi_{2} \,\, &\sim \,\, \pd_{\text{meld}, 1}(\phi_{1}, \psi_{1} \mid Y_{1}), \\ 
  \phi_{2}^{*}, \psi_{1}^{*}, \psi_{2}^{*} \mid \phi_{1} \,\, &\sim \,\, \q(\phi_{2}^{*}, \psi_{1}^{*}, \psi_{2}^{*} \mid \phi_{2}, \psi_{1}, \psi_{2})
  \label{eqn:stage-two-proposals}
\end{align}

==> tex-input/multiple-phi/0030-stage-three-proposals.tex <==
\begin{align}
  \phi_{2}^{*} \mid \psi_{3} \,\, &\sim \,\, \pd_{\text{meld}, 2} (\phi_{1}, \phi_{2}, \psi_{1} \psi_{2} \mid Y_{1}, Y_{2}) \\
  \psi_{3}^{*} \mid \phi_{2} \,\, &\sim \,\, \q(\psi_{3}^{*} \mid \psi_{3})
  \label{eqn:stage-three-proposals}
\end{align}

==> tex-input/multiple-phi/0040-model-ex-dag.tex <==
\begin{figure}[!ht]
  \centering
  \begin{tikzpicture}[node distance = 1.25cm, thick, state/.style={draw = none, minimum width = 1.25cm}]
  % Nodes
  \node [state] (model1) {$\pd_{1}$};
  \node [state][above right = of model1] (model2) {$\pd_{2}$};
  \node [state][below right = of model2] (model3) {$\pd_{3}$};
  \node [state][above right = of model3] (model4) {$\pd_{4}$};
  \node [state][right = of model4] (modelmm1) {$\pd_{\Nm - 1}$};
  \node [state][below right = of modelmm1] (modelM) {$\pd_{\Nm}$};

  % \coordinate [above right = of model2] (blank1);
  % \coordinate [right = of blank1] (blank2);

  % edges with things on them
  \draw (model1) edge node[above left] {$\phi_{1 \cap 2}$} (model2);
  \draw (model2) edge node[above right] {$\phi_{2 \cap 3}$} (model3);
  \draw (model3) edge node[above left] {$\phi_{3 \cap 4}$} (model4);

  \draw [dashed] (model4) edge (modelmm1);

  \draw (modelmm1) edge node[above right] {$\phi_{\Nm - 1 \cap \Nm}$} (modelM);

  \end{tikzpicture}
  \caption{A chain of $\Nm$ models.}
  \label{fig:model-ex-dag}
\end{figure}

==> tex-input/multiple-phi/00501-int-pooled-prior-overall.tex <==
\begin{align}
Z &=
  \int_{\mathbb{R}^{d_{2}}}
  \int_{\mathbb{R}^{d_{1}}} 
    \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}} 
    \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})^{\lambda_{2}}
    \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3}}
  \text{d}\phi_{1 \cap 2}
  \text{d}\phi_{2 \cap 3}   \label{eqn:int-pooled-prior-overall-1} \\
  &=
  \int_{\mathbb{R}^{d_{2}}}
    \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3}}
    \pd_{2}(\phi_{2 \cap 3})^{\lambda_{2}}
  \text{d}\phi_{2 \cap 3}
  \int_{\mathbb{R}^{d_{1}}} 
    \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}} 
    \pd_{2}(\phi_{1 \cap 2} \mid \phi_{2 \cap 3})^{\lambda_{2}}  
  \text{d}\phi_{1 \cap 2}.
     \label{eqn:int-pooled-prior-overall-2}
\end{align}

==> tex-input/multiple-phi/00502-int-pooled-prior-overall-corrected.tex <==
\begin{align}
Z &=
  \int_{\mathbb{R}^{d_{2}}}
  \int_{\mathbb{R}^{d_{1}}} 
    \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}} 
    \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})^{\lambda_{2}}
    \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3}}
  \text{d}\phi_{1 \cap 2}
  \text{d}\phi_{2 \cap 3}   \label{eqn:int-pooled-prior-overall-corrected-1} \\
  &=
  \int_{\mathbb{R}^{d_{2}}}
    \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3}}
    \pd_{2}(\phi_{2 \cap 3})^{\lambda_{2}}
  \left[\int_{\mathbb{R}^{d_{1}}} 
    \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}} 
    \pd_{2}(\phi_{1 \cap 2} \mid \phi_{2 \cap 3})^{\lambda_{2}}  
  \text{d}\phi_{1 \cap 2}
  \right]
  \text{d}\phi_{2 \cap 3}.
     \label{eqn:int-pooled-prior-overall-corrected-2}
\end{align}

==> tex-input/multiple-phi/0051-pooled-prior-overall-general.tex <==
\begin{equation}
  \pd_{\text{pool}} (\phi_{1 \cap 2}, \ldots, \phi_{\Nm - 1 \cap \Nm}) \propto
  \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}} 
  \prod_{\modelindex = 2}^{\Nm - 1} \left\{
    \pd_{\modelindex}(\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1})^{\lambda_{\modelindex}}
  \right\}
  \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm})^{\lambda_{\Nm}}.
  \label{eqn:pooled-prior-overall-general}
\end{equation}

==> tex-input/multiple-phi/0052-linear-pooling.tex <==
\begin{equation}
  \pd_{\text{pool}}(\phi_{1 \cap 2}, \phi_{2 \cap 3}) \propto 
    \lambda_{1} \pd_{1}(\phi_{1 \cap 2}) + 
    \lambda_{2} \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}) + 
    \lambda_{3} \pd_{3}(\phi_{2 \cap 3}).  
  \label{eqn:linear-pooling}
\end{equation}

==> tex-input/multiple-phi/0052-marginal-pooling-weights.tex <==
\begin{equation}
  \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}} = \int \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})^{\lambda_{2}} \text{d}\phi_{2 \cap 3}
  \label{eqn:marginal-pooling-weights}
\end{equation}

==> tex-input/multiple-phi/00521-int-linear-pooling.tex <==
\begin{equation}
Z = \int_{\mathbb{R}^{d_{2}}}
  \int_{\mathbb{R}^{d_{1}}}
  \left[ 
    \lambda_{1} \pd_{1}(\phi_{1 \cap 2}) + 
    \lambda_{2} \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}) + 
    \lambda_{3} \pd_{3}(\phi_{2 \cap 3})
  \right]
  \text{d}\phi_{1 \cap 2}
  \text{d}\phi_{2 \cap 3}
  \label{eqn:int-linear-pooling-1} 
\end{equation}

==> tex-input/multiple-phi/00522-int-linear-pooling.tex <==
\begin{equation}
  \int_{\mathbb{R}^{d_{2}}}
  \text{d}\phi_{2 \cap 3}
  \int_{\mathbb{R}^{d_{1}}} 
    \lambda_{1} \pd_{1}(\phi_{1 \cap 2})
  \text{d}\phi_{1 \cap 2}
  \label{eqn:int-linear-pooling-2}
\end{equation}

==> tex-input/multiple-phi/0053-pooling-via-marginalised-marginals.tex <==
\begin{equation}
  \pd_{\text{pool}} (\phi_{1 \cap 2}, \phi_{2 \cap 3}) \propto
  \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1, 1 \cap 2}}
  \pd_{2}(\phi_{1 \cap 2})^{\lambda_{2, 1 \cap 2}}
  \pd_{2}(\phi_{2 \cap 3})^{\lambda_{2, 2 \cap 3}}
  \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3, 2 \cap 3}}
  \label{eqn:pooling-via-marginalised-marginals}
\end{equation}

==> tex-input/multiple-phi/0054-silly-linear-solution.tex <==
\begin{align}
  \pd_{\text{pool}, 1}(\phi_{1 \cap 2}) &\propto \lambda_{1, 1}\pd_{1}(\phi_{1 \cap 2}) + \lambda_{2, 1}\pd_{2}(\phi_{1 \cap 2}) = \lambda_{1, 1}\pd_{1}(\phi_{1 \cap 2}) + \lambda_{2, 1}\int\pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}) \text{d}\phi_{2 \cap 3} 
  \label{eqn:silly-linear-solution-1}
  \\
  \pd_{\text{pool}, 2}(\phi_{2 \cap 3}) &\propto \lambda_{1, 2}\pd_{2}(\phi_{2 \cap 3}) + \lambda_{2, 2}\pd_{3}(\phi_{2 \cap 3}) = \lambda_{1, 2}\int\pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})\text{d}\phi_{1 \cap 2} + \lambda_{2, 2}\pd_{3}(\phi_{2 \cap 3}),
  \label{eqn:silly-linear-solution-2}
\end{align}

==> tex-input/multiple-phi/00551-linear-normalising-constant.tex <==
\begin{equation}
  K_{\text{lin}}(\lambda) =
    \int
      \prod_{\modelindex = 1}^{\Nm - 1}
      \pd_{\text{pool}, \modelindex}(\phi_{\modelindex \cap \modelindex + 1})
    \text{d}\boldsymbol{\phi},
  \quad \lambda = (\lambda_{1}, \ldots, \lambda_{\Nm}).
\end{equation}



==> tex-input/multiple-phi/0057-dictatorial-pooling.tex <==
\begin{align}
  \pd_{\text{pool, dict}} (\boldsymbol{\phi}) =
    g_{\text{dict}}(\pd_{1}(\phi_{1 \cap 2}), \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}), \pd_{3}(\phi_{2 \cap 3})) &=
    \pd_{1}(\phi_{1 \cap 2}) \pd_{3}(\phi_{2 \cap 3}) \label{eqn:dictatorial-pooling-one} \\
  \pd_{\text{pool, dict}} (\boldsymbol{\phi}) =
    g_{\text{dict}}(\pd_{1}(\phi_{1 \cap 2}), \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}), \pd_{3}(\phi_{2 \cap 3})) &=
    \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}). \label{eqn:dictatorial-pooling-two}
\end{align}

==> tex-input/multiple-phi/0060-pooled-marginals.tex <==
\begin{align}
  \pd_{\text{pool}, 1} (\phi_{1 \cap 2}) &= 
    \int \pd_{\text{pool}} (\phi_{1 \cap 2}, \phi_{2 \cap 3}) \text{d}\phi_{2 \cap 3} 
    \propto
    \int 
      \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}}
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})^{\lambda_{2}}
      \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3}}
    \text{d}\phi_{2 \cap 3} 
    < \infty
    \\
  \pd_{\text{pool}, 2} (\phi_{2 \cap 3}) &= 
    \int \pd_{\text{pool}} (\phi_{1 \cap 2}, \phi_{2 \cap 3}) \text{d}\phi_{1 \cap 2} 
    \propto
    \int 
      \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}}
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})^{\lambda_{2}}
      \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3}}
    \text{d}\phi_{1 \cap 2}
    < \infty.
  \label{eqn:pooled-marginals}
\end{align}

==> tex-input/multiple-phi/0081-M-model-linear-pooling-marg.tex <==
\begin{equation}
  \pd_{\modelindex}(\phi_{\modelindex \cap \modelindex + 1}) = 
  \int \pd_{\modelindex} (\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1}) \text{d}\phi_{\modelindex - 1 \cap \modelindex}.
  \label{eqn:M-model-linear-pooling-marg}
\end{equation}

==> tex-input/multiple-phi/0090-M-model-logarithmic-pooling.tex <==
\begin{equation}
  \pd_{\text{pool}}(\boldsymbol{\phi}) \, \propto \, 
  \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}}
  \prod_{\modelindex = 2}^{\Nm - 2} \left( 
    \pd_{\modelindex}(\phi_{\modelindex - 1\cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1})^{\lambda_{\modelindex}}
  \right)
  \pd_{\Nm}(\phi_{\Nm - 1 \cap \Nm})^{\lambda_{\Nm}}.
  \label{eqn:M-model-logarithmic-pooling}
\end{equation}

==> tex-input/noncommutativity/0005-def-usual-melded-model.tex <==
\begin{align}
  \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \phi_{1}, \psi_{2}, Y_{1}, Y_{2}) 
    &= 
    \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1}) \circledast \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2}) \\
    &=   
    \pd_{\text{pool}}^{12}(\phi_{1 \cap 2})
    \frac{
      \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
    \frac{
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2})
    } {
      \pd_{2}(\phi_{1 \cap 2})
    },
  \label{eqn:def-usual-melded-model}
\end{align}

==> tex-input/noncommutativity/0006-example-melded-marginal-definition.tex <==
\begin{equation}
  \pd_{\text{meld}}^{12}(\phi_{2 \cap 3}) = 
  \int
    \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, Y_{1}, Y_{2})
  \text{d} \left(\boldsymbol{\Theta}_{12} \setminus \phi_{2 \cap 3}\right),
  \label{eqn:example-melded-marginal-definition}
\end{equation}

==> tex-input/noncommutativity/0007-iterated-application-melding.tex <==
\begin{align}
  \pd_{\text{meld}}^{(12)3} (\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, \psi_{3}, Y_{1}, Y_{2}, Y_{3}) 
    &= 
    \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, Y_{1}, Y_{2}) 
    \circledast 
    \pd_{3}(\phi_{2 \cap 3}, \psi_{3}, Y_{3}) 
    \\ &= 
    \pd_{\text{pool}}^{(12)3}(\phi_{2 \cap 3})
    \frac{
      \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, Y_{1}, Y_{2})
    } {
      \pd_{\text{meld}}^{12}(\phi_{2 \cap 3})
    }
    \frac{
      \pd_{3}(\phi_{2 \cap 3}, \psi_{3}, Y_{3})
    } {
      \pd_{3}(\phi_{2 \cap 3})
    }
  \label{eqn:iterated-application-melding-two}
\end{align}

==> tex-input/noncommutativity/0010-usual-melded-model.tex <==
\begin{equation}
  \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, Y_{1}, Y_{2}) = 
    \pd_{\text{pool}}^{12}(\phi_{1 \cap 2})
    \frac{
      \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
    \frac{
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2})
    } {
      \pd_{2}(\phi_{1 \cap 2})
    }.
  \label{eqn:usual-melded-model}
\end{equation}

==> tex-input/noncommutativity/0011-double-melded-model.tex <==
\begin{equation}
  \pd_{\text{meld}}^{(12)3}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, \psi_{3} Y_{1}, Y_{2}, Y_{3}) =
    \pd_{\text{pool}}^{(12)3}(\phi_{2 \cap 3})
    \frac{
      \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, Y_{1}, Y_{2})
    } {
      \pd_{\text{meld}}^{12}(\phi_{2 \cap 3})
    }
    \frac{
      \pd_{3}(\phi_{2 \cap 3}, \psi_{3}, Y_{3})
    } {
      \pd_{3}(\phi_{2 \cap 3})
    },
  \label{eqn:double-melded-model}
\end{equation}

==> tex-input/noncommutativity/0012-strange-marginal-definition.tex <==
\begin{equation}
  \pd_{\text{meld}}^{12}(\phi_{2 \cap 3}) = 
  \int
    \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, Y_{1}, Y_{2})
  \text{d}
  \Omega \setminus \phi_{2 \cap 3}.
  \label{eqn:strange-marginal-definition}
\end{equation}

==> tex-input/noncommutativity/0013-expanded-double-melded-model.tex <==
\begin{multline}
  \pd_{\text{meld}}^{(12)3}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, \psi_{3} Y_{1}, Y_{2}, Y_{3}) = \\
    \pd_{\text{pool}}^{12}(\phi_{1 \cap 2})
    \pd_{\text{pool}}^{(12)3}(\phi_{2 \cap 3}) 
    \frac{
      \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
    \frac {
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2})
    } {
      \pd_{2}(\phi_{1 \cap 2})
      \pd_{\text{meld}}^{12}(\phi_{2 \cap 3})
    }
    \frac{
      \pd_{3}(\phi_{2 \cap 3}, \psi_{3}, Y_{3})
    } {
      \pd_{3}(\phi_{2 \cap 3})
    },
  \label{eqn:expanded-double-melded-model}
\end{multline}

==> tex-input/noncommutativity/0014-orig-melding-commutative-equalities.tex <==
\begin{align}
  \pd_{\text{pool}}^{12}(\phi_{1 \cap 2}) = \pd_{\text{pool}}^{1(23)}(\phi_{1 \cap 2}) \quad &\land \quad
  \pd_{\text{pool}}^{(12)3}(\phi_{2 \cap 3}) = \pd_{\text{pool}}^{23}(\phi_{2 \cap 3}) 
  \label{eqn:orig-melding-commutative-equalities-1}
  \\
  \pd_{2}(\phi_{1 \cap 2}) = \pd_{\text{meld}}^{23}(\phi_{1 \cap 2}) \quad &\land \quad
  \pd_{\text{meld}}^{12}(\phi_{2 \cap 3}) = \pd_{2}(\phi_{2 \cap 3}).
  \label{eqn:orig-melding-commutative-equalities-2}
\end{align}

==> tex-input/noncommutativity/0015-verify-dictatorial-pooling.tex <==
\begin{align}
  \pd_{\text{meld}}^{12}(\phi_{2 \cap 3}) &=
  \int 
    \pd_{\text{meld}}^{12} (\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, Y_{1}, Y_{2}) 
  \text{d} (\boldsymbol{\Theta}_{12} \setminus \phi_{2 \cap 3})
  \\
  &= 
  \int
    \pd_{\text{pool}}^{12}(\phi_{1 \cap 2})
    \frac {
      \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
    \frac {
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2})
    } {
      \pd_{2}(\phi_{1 \cap 2})
    }
  \text{d} (\boldsymbol{\Theta}_{12} \setminus \phi_{2 \cap 3})
  \\
  &=
  \int
    \pd_{\text{pool}}^{12}(\phi_{1 \cap 2})
    \frac {
      \pd_{1}(\phi_{1 \cap 2})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
    \frac {
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})
    } {
      \pd_{2}(\phi_{1 \cap 2})
    }
  \text{d} \phi_{1 \cap 2} \\
  &= 
  \int
    \frac {
      \pd_{\text{pool}}^{12}(\phi_{1 \cap 2})
    } {
      \pd_{2}(\phi_{1 \cap 2})
    }
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})
  \text{d} \phi_{1 \cap 2}.
  \label{eqn:verify-dictatorial-pooling}
\end{align}

==> tex-input/noncommutativity/0016-commutativity-condition.tex <==
\begin{equation}
  \frac {
    \pd_{\text{pool}}^{12}(\phi_{1 \cap 2})
    \pd_{\text{pool}}^{(12)3}(\phi_{2 \cap 3})
  } {
    \pd_{2}(\phi_{1 \cap 2}) 
    \pd_{\text{meld}}^{12}(\phi_{2 \cap 3})
  }
  =
  \frac {
    \pd_{\text{pool}}^{23}(\phi_{2 \cap 3})
    \pd_{\text{pool}}^{1(23)}(\phi_{1 \cap 2})
  } {
    \pd_{\text{meld}}^{23}(\phi_{1 \cap 2}) 
    \pd_{2}(\phi_{2 \cap 3})
  } 
  \label{eqn:commutativity-condition}
\end{equation}

==> tex-input/noncommutativity/0017-pooling-equality.tex <==
\begin{align}
  \pd_{\text{pool}}^{12}(\phi_{1 \cap 2}) 
  &= 
  \pd_{\text{pool}}^{1(23)}(\phi_{1 \cap 2}) 
  \\
  g^{12}(\pd_{1}(\phi_{1 \cap 2}), \pd_{2}(\phi_{1 \cap 2})) 
  &=
  g^{1(23)} (\pd_{1}(\phi_{1 \cap 2}), \pd_{\text{meld}}^{23}(\phi_{1 \cap 2})).
  \label{eqn:pooling-equality}
\end{align}

==> tex-input/noncommutativity/0018-symmetric-expanded-double-melded-model.tex <==
\begin{multline}
  \pd_{\text{meld}}^{1(23)}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, \psi_{2}, \psi_{3} Y_{1}, Y_{2}, Y_{3}) = \\
    \pd_{\text{pool}}^{1(23)}(\phi_{1 \cap 2}) 
    \pd_{\text{pool}}^{23}(\phi_{2 \cap 3})
    \frac{
      \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
    } {
      \pd_{1}(\phi_{1 \cap 2})
    }
    \frac {
      \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{2}, Y_{2})
    } {
      \pd_{\text{meld}}^{23}(\phi_{1 \cap 2})
      \pd_{2}(\phi_{2 \cap 3})
    }
    \frac{
      \pd_{3}(\phi_{2 \cap 3}, \psi_{3}, Y_{3})
    } {
      \pd_{3}(\phi_{2 \cap 3})
    }.
  \label{eqn:symmetric-expanded-double-melded-model}
\end{multline}

==> tex-input/noncommutativity/0020-conditional-commutativity.tex <==
\begin{align}
  \pd_{\text{meld}}^{12} (\phi_{2 \cap 3} \mid A) &= 
    \int
      \pd_{\text{meld}}^{12}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, \psi_{1}, A', Y_{1}, Y_{2} \mid A)
    \text{d} Y_{1}
    \text{d} \psi_{1}
    \text{d} Y_{2}
    \text{d} A'
    \text{d} \phi_{1 \cap 2} \\
  &= 
    \int
      \pd_{\text{pool}}^{12}(\phi_{1 \cap 2} \mid A)
      \frac {
        \pd_{1}(\phi_{1 \cap 2}, \psi_{1}, Y_{1})
      } {
        \pd_{1}(\phi_{1 \cap 2})
      }
      \frac {
        \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}, A', Y_{2} \mid A)
      } {
        \pd_{2}(\phi_{1 \cap 2} \mid A)
      }
    \text{d} Y_{1}
    \text{d} \psi_{1}
    \text{d} Y_{2}
    \text{d} A'
    \text{d} \phi_{1 \cap 2}
  \label{eqn:conditional-commutativity}
\end{align}

==> tex-input/noncommutativity/00201-conditional-commutativity-target-equality.tex <==
\begin{equation}
  \pd_{2}(\phi_{1 \cap 2} \mid A) \pd_{\text{meld}}^{12}(\phi_{2 \cap 3} \mid A) 
  = 
  \pd_{\text{meld}}^{23}(\phi_{1 \cap 2} \mid A) \pd_{2}(\phi_{2 \cap 3} \mid A).
  \label{eqn:conditional-commutativity-target-equality}
\end{equation}

==> tex-input/noncommutativity/0021-conditional-commutativity-two.tex <==
\begin{align}
  &=
    \int
      \pd_{\text{pool}}^{12}(\phi_{1 \cap 2} \mid A)
      \frac {
        \pd_{1}(\phi_{1 \cap 2})
      } {
        \pd_{1}(\phi_{1 \cap 2})
      }
      \frac {
        \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3} \mid A)
      } {
        \pd_{2}(\phi_{1 \cap 2} \mid A)
      }
    \text{d} \phi_{1 \cap 2} 
    \\
  &=
    \pd_{2}(\phi_{2 \cap 3} \mid A)
    \int
       \pd_{\text{pool}}^{12}(\phi_{1 \cap 2} \mid A)
       \frac {
        \pd_{2}(\phi_{1 \cap 2} \mid A)
       } {
        \pd_{2}(\phi_{1 \cap 2} \mid A)
       }
    \text{d} \phi_{1 \cap 2}
    \\
  &= 
    \pd_{2}(\phi_{2 \cap 3} \mid A),
  \label{eqn:conditional-commutativity-two}
\end{align}

==> tex-input/noncommutativity/0030-example-cond-comm.tex <==
\begin{figure}[!hb]
  \centering
  \begin{tikzpicture}[> = stealth, node distance = 1.5cm, thick, state/.style={draw = none, minimum width = 1.25cm}]
  % Model 1 nodes
  \node [state] (m1_psi_1) {$\psi_{1}$};
  \node [state] [below of = m1_psi_1] (m1_phi_12) {$\phi_{1 \cap 2}$};
  \node [state] [below of = m1_phi_12] (m1_Y_1) {$Y_{1}$};

  % Model 2 nodes
  \node [state] [right = 1.3cm of m1_psi_1] (m2_theta_1) {$\theta_{1}$};
  \node [state] [below right = 1.25cm of m2_theta_1] (m2_phi_12) {$\phi_{1 \cap 2}$};
  \node [state] [above right = 1.25cm of m2_phi_12] (m2_theta_2) {$\theta_{2}$};
  \node [state] [below right = 1.25cm of m2_theta_2] (m2_phi_23) {$\phi_{2 \cap 3}$};
  \node [state] [above right = 1.25cm of m2_phi_23] (m2_theta_3) {$\theta_{3}$};
  \node [state] [below right = 1.25cm of m2_phi_12] (m2_Y_2) {$Y_{2}$};

  % Model 3 nodes
  \node [state] [right = 1.3cm of m2_theta_3](m3_psi_3) {$\psi_{3}$};
  \node [state] [below of = m3_psi_3] (m3_phi_23) {$\phi_{2 \cap 3}$};
  \node [state] [below of = m3_phi_23] (m3_Y_3) {$Y_{3}$};

  % Model 1 edges
  \path [->] (m1_psi_1) edge (m1_phi_12);
  \path [->] (m1_phi_12) edge (m1_Y_1);

  % Model 1 bounding box
  \node (m1) [draw = black, fit = (m1_psi_1) (m1_phi_12) (m1_Y_1), dotted] {};
  \node (m1-label) [yshift = -1.5ex] at (m1.south) {$\pd_{1}$};

  % Model 2 edges
  \path [->] (m2_theta_1) edge (m2_phi_12);
  \path [->] (m2_theta_2) edge (m2_phi_12);
  \path [->] (m2_theta_2) edge (m2_phi_23);
  \path [->] (m2_theta_3) edge (m2_phi_23);
  \path [->] (m2_phi_12) edge (m2_Y_2);
  \path [->] (m2_phi_23) edge (m2_Y_2);

  % Model 2 bounding box
  \node (m2) [draw = black, fit = (m2_Y_2) (m2_theta_1) (m2_theta_3), dotted] {};
  \node (m2-label) [yshift = -1.5ex] at (m2.south) {$\pd_{2}$};

  % Model 3 edges
  \path [->] (m3_psi_3) edge (m3_phi_23);
  \path [->] (m3_phi_23) edge (m3_Y_3);

  % Model 3 bounding box
  \node (m3) [draw = black, fit = (m3_psi_3) (m3_phi_23) (m3_Y_3), dotted] {};
  \node (m3-label) [yshift = -1.5ex] at (m3.south) {$\pd_{3}$};

  \end{tikzpicture}
  \caption{An example where the structure of $\pd_{2}$ is such that $\psi_{2} = (\theta_{1}, \theta_{2}, \theta_{3})$,  $A = (\theta_{2})$ and $A' = (\theta_{1}, \theta_{3}).$}
  \label{fig:figure1}
\end{figure}

==> tex-input/noncommutativity/0040-coinciding-equalities.tex <==
\begin{gather}
  \pd_{2}(\phi_{1 \cap 2}) \pd_{\text{meld}}^{12}(\phi_{2 \cap 3}) =
  \pd_{\text{meld}}^{23}(\phi_{1 \cap 2}) \pd_{2}(\phi_{2 \cap 3}) = 
  \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3}) 
  \label{eqn:coinciding-equalities-one}
  \\[1ex]
  \pd_{\text{pool}}^{12}(\phi_{1 \cap 2}) \pd_{\text{pool}}^{(12)3}(\phi_{2 \cap 3}) =
  \pd_{\text{pool}}^{1(23)}(\phi_{1 \cap 2}) \pd_{\text{pool}}^{23}(\phi_{2 \cap 3}) = 
  \pd_{\text{pool}}(\phi_{1 \cap 2}, \phi_{2 \cap 3}).
  \label{eqn:coinciding-equalities-two}
\end{gather}

==> tex-input/noncommutativity/0041-pooling-equality-rhs-log.tex <==
\begin{equation}
  \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1, 1}}
  \pd_{2}(\phi_{1 \cap 2})^{\lambda_{1, 2}}
  \pd_{\text{meld}}^{12}(\phi_{2 \cap 3})^{\lambda_{2, 1}}
  \pd_{3}(\phi_{2 \cap 3})^{\lambda_{2, 1}}
  \, \propto \,
  \pd_{1}(\phi_{1 \cap 2})^{\lambda_{1}} 
  \pd_{2}(\phi_{1 \cap 2}, \phi_{2 \cap 3})^{\lambda_{2}} 
  \pd_{3}(\phi_{2 \cap 3})^{\lambda_{3}},
  \label{eqn:pooling-equality-rhs-log}
\end{equation}

==> tex-input/noncommutativity/0042-pooling-equality-rhs-lin.tex <==
\begin{multline}
  \left(
    \lambda^{'}_{1, 1}\pd_{1}(\phi_{1 \cap 2}) +
    \lambda^{'}_{2, 1}\pd_{2}(\phi_{1 \cap 2}) 
  \right)
  \left(
    \lambda^{'}_{1, 2}\pd_{\text{meld}}^{12}(\phi_{2 \cap 3}) +
    \lambda^{'}_{2, 2}\pd_{3}(\phi_{2 \cap 3})
  \right)
  \, \propto \\
  \left(
    \lambda_{1, 1}\pd_{1}(\phi_{1 \cap 2}) +
    \lambda_{2, 1}\pd_{2}(\phi_{1 \cap 2})
  \right)
  \left(
    \lambda_{1, 2}\pd_{2}(\phi_{2 \cap 3}) +
    \lambda_{2, 2}\pd_{3}(\phi_{2 \cap 3})
  \right).
  \label{eqn:pooling-equality-rhs-lin}
\end{multline}

==> tex-input/owls-example/0050-prior-table.tex <==
\begin{table}[!h]
\centering
\caption{Table of priors for the submodels}
\begin{tabular}{>{\raggedright\arraybackslash}p{2cm}rrrr}
\toprule
Parameter & $\pd_{1}$ & $\pd_{2}$ & $\pd_{3}$ \\
\midrule
\rowcolor{gray!6}  $\alpha$ & $\text{N}_{[-10, 10]}(0, 100^2)$ & $\text{N}_{[-10, 10]}(0, 100^2)$ & Not present \\
$\rho$ & Not present & $\text{U}(0, 10)$ & $\text{U}(0, 10)$ \\
\bottomrule
\end{tabular}
\label{tab:prior_table}
\end{table}

==> tex-input/pooled-prior-discussion/0020-bad-alternative-two.tex <==
\begin{gather}
  \pd_{\text{pool}}(\boldsymbol{\phi}) = 
    \prod_{\modelindex = 1}^{\Nm}
    \pd_{\text{pool}}(\phi_{\modelindex}),
  \quad  \text{where for } \modelindex' = 1 \text{ or } \Nm, \text{ and } \modelindex = 2, \ldots, \Nm - 1 \\
  \pd_{\text{pool}}(\phi_{\modelindex'}) =
    g^{\modelindex'}(\pd_{\modelindex'}(\phi_{\modelindex' \cap \modelindex' + 1}), \pd_{\modelindex' + 1}(\phi_{\modelindex' \cap \modelindex' + 1})),\\
  \pd_{\text{pool}}(\phi_{\modelindex}) =
    g^{\modelindex}(\pd_{\modelindex - 1}(\phi_{\modelindex - 1 \cap \modelindex}), \pd_{\modelindex}(\phi_{\modelindex - 1 \cap \modelindex}, \phi_{\modelindex \cap \modelindex + 1}), \pd_{\modelindex + 1}(\phi_{\modelindex \cap \modelindex + 1}))
  \label{eqn:bad-alterative-one}
\end{gather}

==> tex-input/pooled-prior-discussion/0041-dictatorial-def-all.tex <==
\begin{equation}
\lambda_{\text{dict}} = 
  \begin{cases}
   (\lambda_{1}, 0, \:\ldots\:, 0, \lambda_{\modelindex}, 0, \:\ldots\:, 0, \lambda_{\Nm}) & \text{if $\Nm$ is odd and $\modelindex$ is odd,} \\
   (0, \lambda_{2},  \:\ldots\:, 0, \lambda_{\modelindex}, 0, \:\ldots\:, 0, \lambda_{\Nm - 1}, 0) & \text{if $\Nm$ is odd and $\modelindex$ is even,} \\
   (\lambda_{1}, 0, \:\ldots\:, 0, \lambda_{\modelindex}, 0, \:\ldots\:, 0, \lambda_{\Nm - 1}, 0) & \text{if $\Nm$ is even and $\modelindex$ is odd,} \\
   (0, \lambda_{2}, \:\ldots\:, 0, \lambda_{\modelindex}, 0, \:\ldots\:, 0, \lambda_{\Nm}) & \text{if $\Nm$ is even and $\modelindex$ is even,}
  \end{cases}
  \label{eqn:dictatorial-def-all}
\end{equation}

==> tex-input/pooled-prior-discussion/0042-dictatorial-def-two.tex <==
\begin{equation}
  \pd_{\text{pool, dict}}(\boldsymbol{\phi}) =
  \pd_{1}(\phi_{1 \cap 2})
  \pd_{3}(\phi_{2 \cap 3}, \phi_{3 \cap 4})
  \pd_{5}(\phi_{4 \cap 5}).
  \label{eqn:dictatorial-def-two}
\end{equation}

==> tex-input/pooled-prior-discussion/0044-dictatorial-def-three-part-two.tex <==
\begin{equation}
  \pd_{\text{pool, dict}}(\phi_{\modelindex - 1 \cap \modelindex})
  \pd_{\text{pool, dict}}(\phi_{\modelindex \cap \modelindex + 1}) =
    \pd_{\modelindex}(\phi_{\modelindex - 1 \cap \modelindex})
    \pd_{\modelindex}(\phi_{\modelindex \cap \modelindex + 1})
  \label{eqn:dictatorial-def-three-part-two}
\end{equation}

==> tex-input/pre.tex <==
\usepackage{amsmath,mathtools}
% I always seem to need tikz for something
\usepackage{tikz}
\usetikzlibrary{positioning, shapes, intersections, through, backgrounds, fit, decorations.pathmorphing, angles, quotes}
\usepackage{lineno}
% \linenumbers


\makeatletter
\@ifclassloaded{imsart}{}{
\usepackage{setspace}
\onehalfspacing
}
\makeatother

\usepackage{bbm}

\usepackage{enumitem}
\usepackage{relsize}
\usepackage{placeins}

% required for landscape pages. beware, they back the build very slow.
\usepackage{pdflscape}

% table - `gt' package uses these, often unimportant
\usepackage{longtable}
\usepackage{booktabs}
\usepackage{caption}

\usepackage{color}
\definecolor{myredhighlight}{RGB}{180, 15, 32}
\definecolor{mydarkblue}{RGB}{0, 33, 79}
\definecolor{mymidblue}{RGB}{44, 127, 184}
\definecolor{mylightblue}{RGB}{166, 233, 255}
\definecolor{mygrey}{RGB}{68, 68, 68}

\usepackage{colortbl}

\newcommand{\semitransp}[2][35]{\color{fg!#1}#2}

\setcounter{secnumdepth}{3}

\let\Oldcap\cap
\renewcommand{\cap}{\mathrel{\mathsmaller{\Oldcap}}}

\renewcommand{\floatpagefraction}{0.95}
\renewcommand{\topfraction}{0.95}
\renewcommand{\bottomfraction}{0.95}
\renewcommand{\textfraction}{0.05}

% pd stands for: probability distribution and is useful to distringuish
% marignals for probabilities specifically p(p_{1}) and the like.
\newcommand{\pd}{\text{p}}
\newcommand{\q}{\text{q}}
\newcommand{\w}{\text{w}}
\newcommand{\pdr}{\text{r}}
\newcommand{\pdrh}{\hat{\text{r}}}

% melding
\newcommand{\ppoolphi}{\pd_{\text{pool}}(\phi)}
\newcommand{\pmeld}{\pd_{\text{meld}}}

% the q(x)w(x), "weighted target" density 
% for the moment I'm going to call it s(x), as that is the next letter of the 
% alphabet. Can change it later
\newcommand{\s}{\text{s}}
% direct density estimate - replaces lambda.
\newcommand{\ddest}{\text{s}}
% target weighting function
\newcommand{\tarw}{\text{u}}

% constants - usually sizes of things
\newcommand{\Nx}{N}
\newcommand{\Nnu}{\text{N}_{\text{nu}}}
\newcommand{\Nde}{\text{N}_{\text{de}}}
\newcommand{\Nmc}{\text{N}_{\text{mc}}}
\newcommand{\Nw}{W}
\newcommand{\Nm}{M}
\newcommand{\Ns}{S}
\newcommand{\Np}{P}

% locales - could switch to x and x'
\newcommand{\xnu}{x_{\text{nu}}}
\newcommand{\xde}{x_{\text{de}}}
\newcommand{\phinu}{\phi_{\text{nu}}}
\newcommand{\phide}{\phi_{\text{de}}}

% sugiyama stuff
\newcommand{\pdnu}{\pd_{\text{nu}}}
\newcommand{\pdde}{\pd_{\text{de}}}

% indices 
\newcommand{\wfindex}{w}
\newcommand{\sampleindex}{n}
\newcommand{\modelindex}{m}
\newcommand{\stageindex}{s}
\newcommand{\phiindex}{p}

% independence symbol
\newcommand{\indep}{\perp\!\!\!\perp}
\newcommand{\setcomp}{\mathsf{c}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]

\DeclareMathOperator*{\argmin}{arg\,min}

% ARDS example in text commands
\newcommand{\paoii}{PaO\textsubscript{2}}
\newcommand{\fioii}{FiO\textsubscript{2}}
\newcommand{\spoii}{SpO\textsubscript{2}}
\newcommand{\pfratio}{\paoii/\fioii}
\newcommand{\sfratio}{\spoii/\fioii}


==> tex-input/surv-example/0020-submodel-one-model.tex <==
\begin{equation}
\begin{gathered}
  z_{i, j} = \beta_{0, i} + \beta_{1, i}t_{i, j} + \varepsilon_{i, j} \\
  \beta_{0, i} \sim \text{N}(\mu_{\beta_{0}}, \sigma^{2}_{\beta_{0}}), \,\,
  \beta_{1, i} \sim \text{N}(\mu_{\beta_{1}}, \sigma^{2}_{\beta_{1}}), \,\,
  \varepsilon_{i, j} \sim \text{N}(0, \sigma^{2}_{z}), \\
  \mu_{\beta_{0}} \sim \text{N}(1, 1^2), \,\, 
  \mu_{\beta_{1}} \sim \text{N}(0, 1^2),  \\
  \sigma_{\beta_{0}} \sim \text{LogNormal}(0, 1^2), \,\, 
  \sigma_{\beta_{1}} \sim \text{LogNormal}(1, 1^2), \,\,  
  \sigma_{z} \sim \text{LogNormal}(0, 1^2),
\end{gathered}
\label{eqn:submodel-one-model}
\end{equation}

==> tex-input/surv-example/0030-submodel-two-hazard-general.tex <==
\begin{align}
  h_{i}(t) &= \gamma t^{\gamma - 1} \exp\{\theta_{0} + w_{i}\theta_{1} + \alpha(m_{i}(t))\}, \quad
  S_{i}(t) = \exp\left\{-\int_{0}^{t}h_{i}(u)\text{d}u\right\},
  \label{eqn:submodel-two-hazard-general}
\end{align}

==> tex-input/surv-example/0031-submodel-two-log-likelihood.tex <==
\begin{align}
  \log\pd (T_{i}, d_{i} \mid \boldsymbol{\beta}_{i}, \lambda) &= \mathcal{I}(d_{i} = 1) \log(h_{i}(t)) + 
  \log(S_{i}(t)) \\
  &= \mathcal{I}(d_{i} = 1) \log(h_{i}(t)) - 
  \int_{0}^{t} h_{i}(u) \text{d}u
  \label{eqn:submodel-two-log-likelihood}
\end{align}

==> tex-input/surv-example/0032-submodel-two-hazard-integral.tex <==
\begin{align}
  \int_{0}^{t} h_{i}(u)\text{d}u &=
    \int_{0}^{t} 
      \lambda u ^{\lambda - 1} 
      \exp\{
        \beta_{0, i, k} + \beta_{1, i, k} u
      \} 
    \text{d}u \\
  &=
    \lambda
    \exp\{\beta_{0, i, k}\}
    \frac{\Gamma(\lambda)}{-\beta_{1, i, k}^{\lambda}}
    \int_{0}^{t}
      \frac{-\beta_{1, i, k}^{\lambda}}{\Gamma(\lambda)}
      u^{\lambda - 1}
      \exp\{\beta_{1, i, k} u\}
    \text{d}u \\
  &= 
    \lambda
    \exp\{\beta_{0, i, k}\}
    \frac{\Gamma(\lambda)}{-\beta_{1, i, k}^{\lambda}}
    \frac{1}{\Gamma(\lambda)}
    \gamma(\lambda, -\beta_{1, i k}t) \\
  &=
    -\lambda \beta_{1, i, k}^{-\lambda}
    \exp\{\beta_{0, i, k}\}
    \gamma(\lambda, -\beta_{1, i k}t)
  \label{eqn:submodel-two-hazard-integral}
\end{align}

==> tex-input/surv-example/0033-surv-model-priors.tex <==
\begin{equation}
  \theta_{0} \sim \text{N}(\overline{T}, 1^2), \,\, 
  \theta_{1} \sim \text{N}(0, 1^2), \,\,
  \gamma \sim \text{N}_{+}(0, 1^2), \,\,
  \alpha \sim \text{N}(0, 1^2)
  \label{eqn:surv-model-priors}
\end{equation}

==> tex-input/surv-example/0040-submodel-three-model.tex <==
\begin{equation}
\begin{gathered}
  x_{i, k} = \eta_{0, i} + \eta_{1, i} \tau_{i, k} + \zeta_{i, k}  \\
  \eta_{0, i} \sim \text{N}(\mu_{\eta, 0}, \sigma^{2}_{\eta, 0}), \,\,
  \eta_{0, i} \sim \text{N}(\mu_{\eta, 1}, \sigma^{2}_{\eta, 1}), \,\,
  \zeta_{i, k} \sim \text{N}(0, \sigma^{2}_{x}), \\
  \mu_{\eta, 0} \sim \text{N}(1, 1^2), \,\,
  \mu_{\eta, 1} \sim \text{N}(1, 1^2), \\
  \sigma^{2}_{\eta, 0} \sim \text{LogNormal}(0, 1^2), \,\,
  \sigma^{2}_{\eta, 1} \sim \text{LogNormal}(0, 1^2), \,\,
  \sigma^{2}_{x} \sim \text{LogNormal}(0, 1^2),
\end{gathered}
\label{eqn:submodel-three-model}
\end{equation}

==> tex-input/surv-example/0080-submodel-one-numeric-diags.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{\label{tab:surv-stage-one-submodel-one}Stage one numeric diagnostics for both $\psi_{1}$ and $\phi_{1 \cap 2}$ under submodel 1, in the survival example.}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Stage one numeric diagnostics for both $\psi_{1}$ and $\phi_{1 \cap 2}$ under submodel 1, in the survival example. \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\beta_{0, 1}$} & \cellcolor{gray!6}{0.96} & \cellcolor{gray!6}{0.83} & \cellcolor{gray!6}{1.09} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{23024} & \cellcolor{gray!6}{17665}\\
$\beta_{0, 2}$ & 0.88 & 0.72 & 1.05 & 1 & 23443 & 16033\\
\cellcolor{gray!6}{$\beta_{0, 3}$} & \cellcolor{gray!6}{0.79} & \cellcolor{gray!6}{0.63} & \cellcolor{gray!6}{0.93} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{14511} & \cellcolor{gray!6}{15038}\\
$\beta_{0, 4}$ & 1.04 & 0.86 & 1.25 & 1 & 14932 & 18901\\
\cellcolor{gray!6}{$\beta_{0, 5}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.85} & \cellcolor{gray!6}{1.13} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{19389} & \cellcolor{gray!6}{18920}\\
$\beta_{0, 6}$ & 0.93 & 0.81 & 1.06 & 1 & 24442 & 17799\\
\cellcolor{gray!6}{$\beta_{0, 7}$} & \cellcolor{gray!6}{0.77} & \cellcolor{gray!6}{0.55} & \cellcolor{gray!6}{0.96} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12668} & \cellcolor{gray!6}{11859}\\
$\beta_{0, 8}$ & 0.90 & 0.76 & 1.03 & 1 & 29010 & 17038\\
\cellcolor{gray!6}{$\beta_{0, 9}$} & \cellcolor{gray!6}{0.77} & \cellcolor{gray!6}{0.57} & \cellcolor{gray!6}{0.94} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12015} & \cellcolor{gray!6}{13107}\\
$\beta_{0, 10}$ & 0.88 & 0.73 & 1.02 & 1 & 23043 & 15484\\
\cellcolor{gray!6}{$\beta_{0, 11}$} & \cellcolor{gray!6}{0.91} & \cellcolor{gray!6}{0.76} & \cellcolor{gray!6}{1.06} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24185} & \cellcolor{gray!6}{17149}\\
$\beta_{0, 12}$ & 1.00 & 0.88 & 1.12 & 1 & 19419 & 19827\\
\cellcolor{gray!6}{$\beta_{0, 13}$} & \cellcolor{gray!6}{0.96} & \cellcolor{gray!6}{0.83} & \cellcolor{gray!6}{1.10} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21742} & \cellcolor{gray!6}{17949}\\
$\beta_{0, 14}$ & 0.88 & 0.77 & 1.00 & 1 & 26484 & 19268\\
\cellcolor{gray!6}{$\beta_{0, 15}$} & \cellcolor{gray!6}{0.88} & \cellcolor{gray!6}{0.73} & \cellcolor{gray!6}{1.04} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24110} & \cellcolor{gray!6}{15964}\\
$\beta_{0, 16}$ & 0.96 & 0.78 & 1.16 & 1 & 21034 & 16206\\
\cellcolor{gray!6}{$\beta_{0, 17}$} & \cellcolor{gray!6}{0.89} & \cellcolor{gray!6}{0.73} & \cellcolor{gray!6}{1.06} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22181} & \cellcolor{gray!6}{15773}\\
$\beta_{0, 18}$ & 0.84 & 0.64 & 1.02 & 1 & 18345 & 13455\\
\cellcolor{gray!6}{$\beta_{0, 19}$} & \cellcolor{gray!6}{0.88} & \cellcolor{gray!6}{0.74} & \cellcolor{gray!6}{1.02} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21452} & \cellcolor{gray!6}{17338}\\
$\beta_{0, 20}$ & 0.83 & 0.65 & 1.00 & 1 & 19032 & 14449\\
\cellcolor{gray!6}{$\beta_{0, 21}$} & \cellcolor{gray!6}{0.91} & \cellcolor{gray!6}{0.76} & \cellcolor{gray!6}{1.07} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22343} & \cellcolor{gray!6}{16544}\\
$\beta_{0, 22}$ & 0.93 & 0.77 & 1.09 & 1 & 22935 & 17311\\
\cellcolor{gray!6}{$\beta_{0, 23}$} & \cellcolor{gray!6}{0.85} & \cellcolor{gray!6}{0.69} & \cellcolor{gray!6}{1.01} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{23467} & \cellcolor{gray!6}{15972}\\
$\beta_{0, 24}$ & 0.95 & 0.78 & 1.14 & 1 & 21802 & 17408\\
\cellcolor{gray!6}{$\beta_{0, 25}$} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{0.68} & \cellcolor{gray!6}{0.93} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{20839} & \cellcolor{gray!6}{16243}\\
$\beta_{0, 26}$ & 1.01 & 0.86 & 1.18 & 1 & 17202 & 19009\\
\cellcolor{gray!6}{$\beta_{0, 27}$} & \cellcolor{gray!6}{0.93} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{1.07} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22145} & \cellcolor{gray!6}{17652}\\
$\beta_{0, 28}$ & 0.85 & 0.70 & 0.99 & 1 & 27685 & 15887\\
\cellcolor{gray!6}{$\beta_{0, 29}$} & \cellcolor{gray!6}{0.85} & \cellcolor{gray!6}{0.70} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21302} & \cellcolor{gray!6}{15385}\\
$\beta_{0, 30}$ & 1.01 & 0.85 & 1.20 & 1 & 16290 & 18663\\
\cellcolor{gray!6}{$\beta_{0, 31}$} & \cellcolor{gray!6}{0.82} & \cellcolor{gray!6}{0.61} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{17815} & \cellcolor{gray!6}{14700}\\
$\beta_{0, 32}$ & 0.92 & 0.76 & 1.07 & 1 & 22593 & 16903\\
\cellcolor{gray!6}{$\beta_{0, 33}$} & \cellcolor{gray!6}{0.67} & \cellcolor{gray!6}{0.47} & \cellcolor{gray!6}{0.86} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{8179} & \cellcolor{gray!6}{14140}\\
$\beta_{0, 34}$ & 0.90 & 0.75 & 1.05 & 1 & 27941 & 18288\\
\cellcolor{gray!6}{$\beta_{0, 35}$} & \cellcolor{gray!6}{0.98} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{1.17} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{18186} & \cellcolor{gray!6}{17930}\\
$\beta_{0, 36}$ & 0.89 & 0.76 & 1.02 & 1 & 27973 & 17800\\
\cellcolor{gray!6}{$\beta_{1, 1}$} & \cellcolor{gray!6}{-0.22} & \cellcolor{gray!6}{-0.53} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24033} & \cellcolor{gray!6}{20005}\\
$\beta_{1, 2}$ & -0.71 & -1.02 & -0.40 & 1 & 26325 & 18621\\
\cellcolor{gray!6}{$\beta_{1, 3}$} & \cellcolor{gray!6}{-0.57} & \cellcolor{gray!6}{-0.84} & \cellcolor{gray!6}{-0.29} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{16844} & \cellcolor{gray!6}{17044}\\
$\beta_{1, 4}$ & -0.03 & -0.52 & 0.48 & 1 & 19889 & 20005\\
\cellcolor{gray!6}{$\beta_{1, 5}$} & \cellcolor{gray!6}{-0.37} & \cellcolor{gray!6}{-0.60} & \cellcolor{gray!6}{-0.15} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{23202} & \cellcolor{gray!6}{19454}\\
$\beta_{1, 6}$ & -0.88 & -1.14 & -0.61 & 1 & 24291 & 19537\\
\cellcolor{gray!6}{$\beta_{1, 7}$} & \cellcolor{gray!6}{-0.43} & \cellcolor{gray!6}{-0.82} & \cellcolor{gray!6}{-0.04} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{17776} & \cellcolor{gray!6}{14256}\\
$\beta_{1, 8}$ & -0.29 & -0.74 & 0.17 & 1 & 29019 & 19477\\
\cellcolor{gray!6}{$\beta_{1, 9}$} & \cellcolor{gray!6}{-0.94} & \cellcolor{gray!6}{-1.38} & \cellcolor{gray!6}{-0.50} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{16813} & \cellcolor{gray!6}{14731}\\
$\beta_{1, 10}$ & -0.90 & -1.11 & -0.68 & 1 & 23579 & 16244\\
\cellcolor{gray!6}{$\beta_{1, 11}$} & \cellcolor{gray!6}{-0.64} & \cellcolor{gray!6}{-0.90} & \cellcolor{gray!6}{-0.38} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25065} & \cellcolor{gray!6}{17926}\\
$\beta_{1, 12}$ & -0.82 & -1.07 & -0.56 & 1 & 23650 & 19680\\
\cellcolor{gray!6}{$\beta_{1, 13}$} & \cellcolor{gray!6}{-0.51} & \cellcolor{gray!6}{-0.90} & \cellcolor{gray!6}{-0.12} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25219} & \cellcolor{gray!6}{19171}\\
$\beta_{1, 14}$ & -0.31 & -0.51 & -0.12 & 1 & 28260 & 19079\\
\cellcolor{gray!6}{$\beta_{1, 15}$} & \cellcolor{gray!6}{-0.73} & \cellcolor{gray!6}{-1.04} & \cellcolor{gray!6}{-0.42} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25070} & \cellcolor{gray!6}{19395}\\
$\beta_{1, 16}$ & -0.34 & -0.71 & 0.03 & 1 & 23974 & 19593\\
\cellcolor{gray!6}{$\beta_{1, 17}$} & \cellcolor{gray!6}{-0.68} & \cellcolor{gray!6}{-1.00} & \cellcolor{gray!6}{-0.36} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25015} & \cellcolor{gray!6}{19397}\\
$\beta_{1, 18}$ & -0.77 & -1.16 & -0.39 & 1 & 20699 & 17444\\
\cellcolor{gray!6}{$\beta_{1, 19}$} & \cellcolor{gray!6}{-0.12} & \cellcolor{gray!6}{-0.34} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22533} & \cellcolor{gray!6}{18234}\\
$\beta_{1, 20}$ & -0.70 & -1.06 & -0.34 & 1 & 25806 & 18804\\
\cellcolor{gray!6}{$\beta_{1, 21}$} & \cellcolor{gray!6}{-0.86} & \cellcolor{gray!6}{-1.17} & \cellcolor{gray!6}{-0.55} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22289} & \cellcolor{gray!6}{19219}\\
$\beta_{1, 22}$ & -0.91 & -1.27 & -0.56 & 1 & 24969 & 18785\\
\cellcolor{gray!6}{$\beta_{1, 23}$} & \cellcolor{gray!6}{-0.69} & \cellcolor{gray!6}{-1.00} & \cellcolor{gray!6}{-0.37} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{28003} & \cellcolor{gray!6}{20604}\\
$\beta_{1, 24}$ & -0.22 & -0.55 & 0.11 & 1 & 21255 & 18812\\
\cellcolor{gray!6}{$\beta_{1, 25}$} & \cellcolor{gray!6}{-0.66} & \cellcolor{gray!6}{-0.95} & \cellcolor{gray!6}{-0.38} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{30061} & \cellcolor{gray!6}{19000}\\
$\beta_{1, 26}$ & -0.37 & -0.65 & -0.09 & 1 & 22495 & 19433\\
\cellcolor{gray!6}{$\beta_{1, 27}$} & \cellcolor{gray!6}{-0.75} & \cellcolor{gray!6}{-1.07} & \cellcolor{gray!6}{-0.43} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24383} & \cellcolor{gray!6}{19407}\\
$\beta_{1, 28}$ & -0.58 & -1.15 & -0.02 & 1 & 33261 & 19282\\
\cellcolor{gray!6}{$\beta_{1, 29}$} & \cellcolor{gray!6}{-0.57} & \cellcolor{gray!6}{-0.80} & \cellcolor{gray!6}{-0.33} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21516} & \cellcolor{gray!6}{17923}\\
$\beta_{1, 30}$ & -0.31 & -0.63 & -0.01 & 1 & 19680 & 19535\\
\cellcolor{gray!6}{$\beta_{1, 31}$} & \cellcolor{gray!6}{-0.86} & \cellcolor{gray!6}{-1.20} & \cellcolor{gray!6}{-0.51} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{20872} & \cellcolor{gray!6}{17547}\\
$\beta_{1, 32}$ & -0.23 & -0.51 & 0.05 & 1 & 22445 & 17906\\
\cellcolor{gray!6}{$\beta_{1, 33}$} & \cellcolor{gray!6}{-0.08} & \cellcolor{gray!6}{-0.44} & \cellcolor{gray!6}{0.29} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12460} & \cellcolor{gray!6}{15855}\\
$\beta_{1, 34}$ & -0.57 & -1.00 & -0.13 & 1 & 30443 & 19270\\
\cellcolor{gray!6}{$\beta_{1, 35}$} & \cellcolor{gray!6}{-0.19} & \cellcolor{gray!6}{-0.50} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{19888} & \cellcolor{gray!6}{17643}\\
$\beta_{1, 36}$ & -0.44 & -0.72 & -0.16 & 1 & 29313 & 19708\\
\cellcolor{gray!6}{$\mu_{\beta, 0}$} & \cellcolor{gray!6}{0.89} & \cellcolor{gray!6}{0.84} & \cellcolor{gray!6}{0.95} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{10765} & \cellcolor{gray!6}{16101}\\
$\mu_{\beta, 1}$ & -0.53 & -0.66 & -0.40 & 1 & 14410 & 18454\\
\cellcolor{gray!6}{$\sigma_{\beta, 0}$} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4777} & \cellcolor{gray!6}{5979}\\
$\sigma_{\beta, 1}$ & 0.35 & 0.25 & 0.46 & 1 & 13868 & 14638\\
\cellcolor{gray!6}{$\sigma_{y}$} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{15022} & \cellcolor{gray!6}{19497}\\*
\end{longtable}

==> tex-input/surv-example/0081-submodel-three-numeric-diags.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{\label{tab:surv-stage-one-submodel-three}Stage one numeric diagnostics for both $\psi_{3}$ and $\phi_{2 \cap 3}$ under submodel 3, in the survival example.}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Stage one numeric diagnostics for both $\psi_{3}$ and $\phi_{2 \cap 3}$ under submodel 3, in the survival example. \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\mu_{\eta, 0}$} & \cellcolor{gray!6}{1.89} & \cellcolor{gray!6}{1.51} & \cellcolor{gray!6}{2.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{14434} & \cellcolor{gray!6}{18892}\\
$\mu_{\eta, 1}$ & 0.72 & 0.10 & 1.36 & 1 & 11782 & 18081\\
\cellcolor{gray!6}{$\sigma_{\eta, 0}$} & \cellcolor{gray!6}{1.07} & \cellcolor{gray!6}{0.74} & \cellcolor{gray!6}{1.43} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{10210} & \cellcolor{gray!6}{11156}\\
$\sigma_{\eta, 1}$ & 1.61 & 0.96 & 2.31 & 1 & 5554 & 4869\\
\cellcolor{gray!6}{$\eta_{1,  0}$} & \cellcolor{gray!6}{0.58} & \cellcolor{gray!6}{-0.27} & \cellcolor{gray!6}{1.43} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{26281} & \cellcolor{gray!6}{19156}\\
$\eta_{2,  0}$ & 1.47 & 0.32 & 2.60 & 1 & 24745 & 19527\\
\cellcolor{gray!6}{$\eta_{3,  0}$} & \cellcolor{gray!6}{3.23} & \cellcolor{gray!6}{2.25} & \cellcolor{gray!6}{4.21} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{14827} & \cellcolor{gray!6}{18305}\\
$\eta_{4,  0}$ & 1.97 & 0.67 & 3.25 & 1 & 23944 & 20305\\
\cellcolor{gray!6}{$\eta_{5,  0}$} & \cellcolor{gray!6}{1.23} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{2.29} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21723} & \cellcolor{gray!6}{18811}\\
$\eta_{6,  0}$ & 1.03 & 0.23 & 1.83 & 1 & 27077 & 20506\\
\cellcolor{gray!6}{$\eta_{7,  0}$} & \cellcolor{gray!6}{4.03} & \cellcolor{gray!6}{2.65} & \cellcolor{gray!6}{5.42} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{13188} & \cellcolor{gray!6}{15171}\\
$\eta_{8,  0}$ & 1.72 & 0.66 & 2.76 & 1 & 28731 & 20486\\
\cellcolor{gray!6}{$\eta_{9,  0}$} & \cellcolor{gray!6}{1.13} & \cellcolor{gray!6}{0.24} & \cellcolor{gray!6}{2.02} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{32704} & \cellcolor{gray!6}{20594}\\
$\eta_{10,  0}$ & 1.35 & 0.71 & 2.00 & 1 & 30092 & 19869\\
\cellcolor{gray!6}{$\eta_{11,  0}$} & \cellcolor{gray!6}{2.20} & \cellcolor{gray!6}{1.41} & \cellcolor{gray!6}{2.99} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{26539} & \cellcolor{gray!6}{21003}\\
$\eta_{12,  0}$ & 2.55 & 1.53 & 3.56 & 1 & 15545 & 16448\\
\cellcolor{gray!6}{$\eta_{13,  0}$} & \cellcolor{gray!6}{2.21} & \cellcolor{gray!6}{1.29} & \cellcolor{gray!6}{3.13} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{27142} & \cellcolor{gray!6}{19730}\\
$\eta_{14,  0}$ & 1.23 & 0.16 & 2.30 & 1 & 20698 & 19324\\
\cellcolor{gray!6}{$\eta_{15,  0}$} & \cellcolor{gray!6}{1.11} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{2.02} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{27804} & \cellcolor{gray!6}{20001}\\
$\eta_{16,  0}$ & 1.01 & -0.19 & 2.19 & 1 & 26563 & 18964\\
\cellcolor{gray!6}{$\eta_{17,  0}$} & \cellcolor{gray!6}{1.62} & \cellcolor{gray!6}{0.76} & \cellcolor{gray!6}{2.48} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{29577} & \cellcolor{gray!6}{20050}\\
$\eta_{18,  0}$ & 2.15 & 0.92 & 3.39 & 1 & 25588 & 19727\\
\cellcolor{gray!6}{$\eta_{19,  0}$} & \cellcolor{gray!6}{1.53} & \cellcolor{gray!6}{0.78} & \cellcolor{gray!6}{2.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{23475} & \cellcolor{gray!6}{19586}\\
$\eta_{20,  0}$ & 2.34 & 1.11 & 3.62 & 1 & 12504 & 13856\\
\cellcolor{gray!6}{$\eta_{21,  0}$} & \cellcolor{gray!6}{3.13} & \cellcolor{gray!6}{2.27} & \cellcolor{gray!6}{3.99} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24809} & \cellcolor{gray!6}{19186}\\
$\eta_{22,  0}$ & 1.81 & 0.73 & 2.88 & 1 & 27111 & 19991\\
\cellcolor{gray!6}{$\eta_{23,  0}$} & \cellcolor{gray!6}{2.22} & \cellcolor{gray!6}{0.92} & \cellcolor{gray!6}{3.53} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22125} & \cellcolor{gray!6}{19863}\\
$\eta_{24,  0}$ & 2.00 & 0.82 & 3.19 & 1 & 25002 & 19116\\
\cellcolor{gray!6}{$\eta_{25,  0}$} & \cellcolor{gray!6}{2.97} & \cellcolor{gray!6}{1.93} & \cellcolor{gray!6}{4.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{17267} & \cellcolor{gray!6}{18883}\\
$\eta_{26,  0}$ & 1.23 & 0.23 & 2.21 & 1 & 26162 & 20442\\
\cellcolor{gray!6}{$\eta_{27,  0}$} & \cellcolor{gray!6}{1.40} & \cellcolor{gray!6}{0.55} & \cellcolor{gray!6}{2.25} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{29489} & \cellcolor{gray!6}{19512}\\
$\eta_{28,  0}$ & 2.83 & 1.52 & 4.18 & 1 & 14415 & 16388\\
\cellcolor{gray!6}{$\eta_{29,  0}$} & \cellcolor{gray!6}{1.65} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{2.30} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{30901} & \cellcolor{gray!6}{21277}\\
$\eta_{30,  0}$ & 1.05 & -0.10 & 2.20 & 1 & 23792 & 19190\\
\cellcolor{gray!6}{$\eta_{31,  0}$} & \cellcolor{gray!6}{2.35} & \cellcolor{gray!6}{1.19} & \cellcolor{gray!6}{3.51} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{26209} & \cellcolor{gray!6}{18625}\\
$\eta_{32,  0}$ & 1.47 & 0.42 & 2.51 & 1 & 24976 & 19448\\
\cellcolor{gray!6}{$\eta_{33,  0}$} & \cellcolor{gray!6}{3.94} & \cellcolor{gray!6}{2.65} & \cellcolor{gray!6}{5.18} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12412} & \cellcolor{gray!6}{13985}\\
$\eta_{34,  0}$ & 3.08 & 2.21 & 3.96 & 1 & 26190 & 18902\\
\cellcolor{gray!6}{$\eta_{35,  0}$} & \cellcolor{gray!6}{1.51} & \cellcolor{gray!6}{0.40} & \cellcolor{gray!6}{2.59} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24300} & \cellcolor{gray!6}{19792}\\
$\eta_{36,  0}$ & 0.92 & -0.12 & 1.94 & 1 & 23972 & 19893\\
\cellcolor{gray!6}{$\eta_{1,  1}$} & \cellcolor{gray!6}{0.40} & \cellcolor{gray!6}{-1.16} & \cellcolor{gray!6}{1.93} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{26821} & \cellcolor{gray!6}{18974}\\
$\eta_{2,  1}$ & 0.44 & -1.65 & 2.54 & 1 & 25592 & 20001\\
\cellcolor{gray!6}{$\eta_{3,  1}$} & \cellcolor{gray!6}{2.10} & \cellcolor{gray!6}{0.42} & \cellcolor{gray!6}{3.87} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{13884} & \cellcolor{gray!6}{17298}\\
$\eta_{4,  1}$ & -0.02 & -1.82 & 1.74 & 1 & 24628 & 20732\\
\cellcolor{gray!6}{$\eta_{5,  1}$} & \cellcolor{gray!6}{-0.73} & \cellcolor{gray!6}{-2.69} & \cellcolor{gray!6}{1.11} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{19865} & \cellcolor{gray!6}{18555}\\
$\eta_{6,  1}$ & 0.63 & -0.77 & 2.07 & 1 & 27791 & 21465\\
\cellcolor{gray!6}{$\eta_{7,  1}$} & \cellcolor{gray!6}{2.44} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{5.14} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{11960} & \cellcolor{gray!6}{16274}\\
$\eta_{8,  1}$ & 0.14 & -1.44 & 1.69 & 1 & 28911 & 20709\\
\cellcolor{gray!6}{$\eta_{9,  1}$} & \cellcolor{gray!6}{-0.14} & \cellcolor{gray!6}{-2.74} & \cellcolor{gray!6}{2.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{26992} & \cellcolor{gray!6}{18502}\\
$\eta_{10,  1}$ & -0.18 & -1.58 & 1.18 & 1 & 26803 & 20192\\
\cellcolor{gray!6}{$\eta_{11,  1}$} & \cellcolor{gray!6}{-0.86} & \cellcolor{gray!6}{-2.22} & \cellcolor{gray!6}{0.50} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22292} & \cellcolor{gray!6}{20113}\\
$\eta_{12,  1}$ & -2.05 & -3.77 & -0.32 & 1 & 13164 & 12199\\
\cellcolor{gray!6}{$\eta_{13,  1}$} & \cellcolor{gray!6}{1.11} & \cellcolor{gray!6}{-0.30} & \cellcolor{gray!6}{2.57} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24740} & \cellcolor{gray!6}{19483}\\
$\eta_{14,  1}$ & -0.69 & -2.26 & 0.85 & 1 & 19821 & 19582\\
\cellcolor{gray!6}{$\eta_{15,  1}$} & \cellcolor{gray!6}{0.33} & \cellcolor{gray!6}{-1.95} & \cellcolor{gray!6}{2.53} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{26349} & \cellcolor{gray!6}{19536}\\
$\eta_{16,  1}$ & 0.35 & -1.62 & 2.27 & 1 & 27986 & 19210\\
\cellcolor{gray!6}{$\eta_{17,  1}$} & \cellcolor{gray!6}{1.23} & \cellcolor{gray!6}{-0.42} & \cellcolor{gray!6}{2.94} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{28949} & \cellcolor{gray!6}{19136}\\
$\eta_{18,  1}$ & 0.63 & -1.49 & 2.75 & 1 & 25010 & 19428\\
\cellcolor{gray!6}{$\eta_{19,  1}$} & \cellcolor{gray!6}{1.74} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{3.42} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{18872} & \cellcolor{gray!6}{19508}\\
$\eta_{20,  1}$ & 3.83 & 1.54 & 6.14 & 1 & 8619 & 8452\\
\cellcolor{gray!6}{$\eta_{21,  1}$} & \cellcolor{gray!6}{-0.04} & \cellcolor{gray!6}{-2.05} & \cellcolor{gray!6}{1.90} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25837} & \cellcolor{gray!6}{18119}\\
$\eta_{22,  1}$ & 1.28 & -0.45 & 3.05 & 1 & 24452 & 19513\\
\cellcolor{gray!6}{$\eta_{23,  1}$} & \cellcolor{gray!6}{1.39} & \cellcolor{gray!6}{-0.52} & \cellcolor{gray!6}{3.40} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22193} & \cellcolor{gray!6}{19337}\\
$\eta_{24,  1}$ & 0.33 & -1.28 & 1.93 & 1 & 24363 & 19312\\
\cellcolor{gray!6}{$\eta_{25,  1}$} & \cellcolor{gray!6}{1.74} & \cellcolor{gray!6}{-0.22} & \cellcolor{gray!6}{3.80} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{15355} & \cellcolor{gray!6}{19096}\\
$\eta_{26,  1}$ & 0.99 & -0.53 & 2.55 & 1 & 26326 & 19271\\
\cellcolor{gray!6}{$\eta_{27,  1}$} & \cellcolor{gray!6}{0.94} & \cellcolor{gray!6}{-0.47} & \cellcolor{gray!6}{2.36} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{29327} & \cellcolor{gray!6}{19600}\\
$\eta_{28,  1}$ & 2.85 & 0.91 & 4.82 & 1 & 11406 & 14071\\
\cellcolor{gray!6}{$\eta_{29,  1}$} & \cellcolor{gray!6}{-0.49} & \cellcolor{gray!6}{-1.76} & \cellcolor{gray!6}{0.78} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25509} & \cellcolor{gray!6}{18934}\\
$\eta_{30,  1}$ & 0.03 & -1.54 & 1.57 & 1 & 25107 & 19484\\
\cellcolor{gray!6}{$\eta_{31,  1}$} & \cellcolor{gray!6}{1.33} & \cellcolor{gray!6}{-0.88} & \cellcolor{gray!6}{3.67} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{23575} & \cellcolor{gray!6}{19151}\\
$\eta_{32,  1}$ & -0.20 & -1.79 & 1.37 & 1 & 24531 & 19940\\
\cellcolor{gray!6}{$\eta_{33,  1}$} & \cellcolor{gray!6}{2.74} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{5.98} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{10830} & \cellcolor{gray!6}{14500}\\
$\eta_{34,  1}$ & 1.37 & -1.23 & 4.23 & 1 & 22201 & 16111\\
\cellcolor{gray!6}{$\eta_{35,  1}$} & \cellcolor{gray!6}{0.75} & \cellcolor{gray!6}{-0.88} & \cellcolor{gray!6}{2.44} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25014} & \cellcolor{gray!6}{18186}\\
$\eta_{36,  1}$ & -0.36 & -1.93 & 1.18 & 1 & 23367 & 19000\\
\cellcolor{gray!6}{$\sigma_{y}$} & \cellcolor{gray!6}{0.90} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{1.01} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{18498} & \cellcolor{gray!6}{17938}\\*
\end{longtable}

==> tex-input/surv-example/0090-stage-two-phi-12-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{\label{tab:surv-stage-two-diag-phi-12}Stage two numeric diagnostics for $\phi_{1 \cap 2}$ in the survival example}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Stage two numeric diagnostics for $\phi_{1 \cap 2}$ in the survival example \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$t_{1}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25010} & \cellcolor{gray!6}{24995}\\
$t_{2}$ & 0.97 & 0.82 & 1.00 & 1 & 9381 & 24995\\
\cellcolor{gray!6}{$t_{3}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.90} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{10535} & \cellcolor{gray!6}{24995}\\
$t_{4}$ & 1.00 & 1.00 & 1.00 & 1 & 14192 & 24995\\
\cellcolor{gray!6}{$t_{5}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$t_{6}$ & 0.91 & 0.75 & 1.00 & 1 & 6282 & 24995\\
\cellcolor{gray!6}{$t_{7}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.98} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{15884} & \cellcolor{gray!6}{24995}\\
$t_{8}$ & 1.00 & 1.00 & 1.00 & 1 & 19594 & 24995\\
\cellcolor{gray!6}{$t_{9}$} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{0.56} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{2312} & \cellcolor{gray!6}{24995}\\
$t_{10}$ & 0.80 & 0.69 & 0.94 & 1 & 4913 & 3235\\
\cellcolor{gray!6}{$t_{11}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.91} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{13728} & \cellcolor{gray!6}{24995}\\
$t_{12}$ & 0.95 & 0.82 & 1.00 & 1 & 9366 & 24995\\
\cellcolor{gray!6}{$t_{13}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21494} & \cellcolor{gray!6}{24995}\\
$t_{14}$ & 1.00 & 1.00 & 1.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$t_{15}$} & \cellcolor{gray!6}{0.96} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{8495} & \cellcolor{gray!6}{24995}\\
$t_{16}$ & 1.00 & 1.00 & 1.00 & 1 & 13357 & 24995\\
\cellcolor{gray!6}{$t_{17}$} & \cellcolor{gray!6}{0.98} & \cellcolor{gray!6}{0.88} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{13095} & \cellcolor{gray!6}{24995}\\
$t_{18}$ & 0.94 & 0.73 & 1.00 & 1 & 6502 & 24995\\
\cellcolor{gray!6}{$t_{19}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$t_{20}$ & 0.98 & 0.85 & 1.00 & 1 & 6003 & 24995\\
\cellcolor{gray!6}{$t_{21}$} & \cellcolor{gray!6}{0.91} & \cellcolor{gray!6}{0.74} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{7691} & \cellcolor{gray!6}{24995}\\
$t_{22}$ & 0.93 & 0.73 & 1.00 & 1 & 4776 & 24995\\
\cellcolor{gray!6}{$t_{23}$} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{0.83} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{9624} & \cellcolor{gray!6}{24995}\\
$t_{24}$ & 1.00 & 1.00 & 1.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$t_{25}$} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{0.82} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{7967} & \cellcolor{gray!6}{24995}\\
$t_{26}$ & 1.00 & 1.00 & 1.00 & 1 & 25014 & 24995\\
\cellcolor{gray!6}{$t_{27}$} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{0.84} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{11491} & \cellcolor{gray!6}{24995}\\
$t_{28}$ & 0.99 & 0.94 & 1.00 & 1 & 10056 & 24995\\
\cellcolor{gray!6}{$t_{29}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.93} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{15196} & \cellcolor{gray!6}{24995}\\
$t_{30}$ & 1.00 & 1.00 & 1.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$t_{31}$} & \cellcolor{gray!6}{0.88} & \cellcolor{gray!6}{0.66} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{3341} & \cellcolor{gray!6}{24995}\\
$t_{32}$ & 1.00 & 1.00 & 1.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$t_{33}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21894} & \cellcolor{gray!6}{24995}\\
$t_{34}$ & 0.99 & 0.92 & 1.00 & 1 & 13558 & 24995\\
\cellcolor{gray!6}{$t_{35}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$t_{36}$ & 1.00 & 1.00 & 1.00 & 1 & 14770 & 24995\\
\cellcolor{gray!6}{$\delta_{1}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25010} & \cellcolor{gray!6}{25010}\\
$\delta_{2}$ & 0.35 & 0.00 & 1.00 & 1 & 8642 & 24995\\
\cellcolor{gray!6}{$\delta_{3}$} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{9952} & \cellcolor{gray!6}{24995}\\
$\delta_{4}$ & 0.00 & 0.00 & 0.00 & 1 & 13891 & 13891\\
\cellcolor{gray!6}{$\delta_{5}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$\delta_{6}$ & 0.69 & 0.00 & 1.00 & 1 & 4651 & 24995\\
\cellcolor{gray!6}{$\delta_{7}$} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{15574} & \cellcolor{gray!6}{24995}\\
$\delta_{8}$ & 0.03 & 0.00 & 0.00 & 1 & 19519 & 19519\\
\cellcolor{gray!6}{$\delta_{9}$} & \cellcolor{gray!6}{0.83} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{1776} & \cellcolor{gray!6}{24995}\\
$\delta_{10}$ & 0.99 & 1.00 & 1.00 & 1 & 4125 & 24995\\
\cellcolor{gray!6}{$\delta_{11}$} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12745} & \cellcolor{gray!6}{24995}\\
$\delta_{12}$ & 0.64 & 0.00 & 1.00 & 1 & 9227 & 24995\\
\cellcolor{gray!6}{$\delta_{13}$} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21219} & \cellcolor{gray!6}{21219}\\
$\delta_{14}$ & 0.00 & 0.00 & 0.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$\delta_{15}$} & \cellcolor{gray!6}{0.44} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{7732} & \cellcolor{gray!6}{24995}\\
$\delta_{16}$ & 0.01 & 0.00 & 0.00 & 1 & 12557 & 12557\\
\cellcolor{gray!6}{$\delta_{17}$} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12408} & \cellcolor{gray!6}{24995}\\
$\delta_{18}$ & 0.47 & 0.00 & 1.00 & 1 & 5542 & 24995\\
\cellcolor{gray!6}{$\delta_{19}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$\delta_{20}$ & 0.15 & 0.00 & 1.00 & 1 & 5759 & 24995\\
\cellcolor{gray!6}{$\delta_{21}$} & \cellcolor{gray!6}{0.73} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5658} & \cellcolor{gray!6}{24995}\\
$\delta_{22}$ & 0.53 & 0.00 & 1.00 & 1 & 3899 & 24995\\
\cellcolor{gray!6}{$\delta_{23}$} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{9102} & \cellcolor{gray!6}{24995}\\
$\delta_{24}$ & 0.00 & 0.00 & 0.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$\delta_{25}$} & \cellcolor{gray!6}{0.27} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{7342} & \cellcolor{gray!6}{24995}\\
$\delta_{26}$ & 0.00 & 0.00 & 0.00 & 1 & 25014 & 25014\\
\cellcolor{gray!6}{$\delta_{27}$} & \cellcolor{gray!6}{0.28} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{10629} & \cellcolor{gray!6}{24995}\\
$\delta_{28}$ & 0.08 & 0.00 & 1.00 & 1 & 9972 & 24995\\
\cellcolor{gray!6}{$\delta_{29}$} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{13883} & \cellcolor{gray!6}{24995}\\
$\delta_{30}$ & 0.00 & 0.00 & 0.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$\delta_{31}$} & \cellcolor{gray!6}{0.67} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{2484} & \cellcolor{gray!6}{24995}\\
$\delta_{32}$ & 0.00 & 0.00 & 0.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$\delta_{33}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21870} & \cellcolor{gray!6}{21870}\\
$\delta_{34}$ & 0.10 & 0.00 & 1.00 & 1 & 12552 & 24995\\
\cellcolor{gray!6}{$\delta_{35}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$\delta_{36}$ & 0.03 & 0.00 & 0.00 & 1 & 14178 & 14178\\*
\end{longtable}

==> tex-input/surv-example/0091-stage-two-phi-23-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{\label{tab:surv-stage-two-diag-phi-23}Stage two numeric diagnostics for $\phi_{2 \cap 3}$ in the survival example}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Stage two numeric diagnostics for $\phi_{2 \cap 3}$ in the survival example \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\eta_{1, 0}$} & \cellcolor{gray!6}{0.59} & \cellcolor{gray!6}{-0.26} & \cellcolor{gray!6}{1.44} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5429} & \cellcolor{gray!6}{4249}\\
$\eta_{2, 0}$ & 1.50 & 0.29 & 2.67 & 1 & 4250 & 2584\\
\cellcolor{gray!6}{$\eta_{3, 0}$} & \cellcolor{gray!6}{3.21} & \cellcolor{gray!6}{2.24} & \cellcolor{gray!6}{4.17} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5068} & \cellcolor{gray!6}{3813}\\
$\eta_{4, 0}$ & 2.01 & 0.69 & 3.31 & 1 & 5205 & 4553\\
\cellcolor{gray!6}{$\eta_{5, 0}$} & \cellcolor{gray!6}{1.24} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{2.32} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4994} & \cellcolor{gray!6}{4274}\\
$\eta_{6, 0}$ & 1.05 & 0.23 & 1.84 & 1 & 4904 & 3868\\
\cellcolor{gray!6}{$\eta_{7, 0}$} & \cellcolor{gray!6}{4.01} & \cellcolor{gray!6}{2.56} & \cellcolor{gray!6}{5.40} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4033} & \cellcolor{gray!6}{2731}\\
$\eta_{8, 0}$ & 1.73 & 0.69 & 2.74 & 1 & 5050 & 5221\\
\cellcolor{gray!6}{$\eta_{9, 0}$} & \cellcolor{gray!6}{1.15} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{2.04} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5102} & \cellcolor{gray!6}{3998}\\
$\eta_{10, 0}$ & 1.37 & 0.72 & 1.99 & 1 & 6196 & 6536\\
\cellcolor{gray!6}{$\eta_{11, 0}$} & \cellcolor{gray!6}{2.23} & \cellcolor{gray!6}{1.43} & \cellcolor{gray!6}{3.02} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5797} & \cellcolor{gray!6}{4961}\\
$\eta_{12, 0}$ & 2.57 & 1.53 & 3.59 & 1 & 5211 & 4799\\
\cellcolor{gray!6}{$\eta_{13, 0}$} & \cellcolor{gray!6}{2.20} & \cellcolor{gray!6}{1.27} & \cellcolor{gray!6}{3.12} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4651} & \cellcolor{gray!6}{3864}\\
$\eta_{14, 0}$ & 1.25 & 0.15 & 2.32 & 1 & 5075 & 4267\\
\cellcolor{gray!6}{$\eta_{15, 0}$} & \cellcolor{gray!6}{1.14} & \cellcolor{gray!6}{0.24} & \cellcolor{gray!6}{2.08} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5216} & \cellcolor{gray!6}{3867}\\
$\eta_{16, 0}$ & 1.03 & -0.15 & 2.19 & 1 & 5367 & 5397\\
\cellcolor{gray!6}{$\eta_{17, 0}$} & \cellcolor{gray!6}{1.63} & \cellcolor{gray!6}{0.76} & \cellcolor{gray!6}{2.48} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4869} & \cellcolor{gray!6}{4784}\\
$\eta_{18, 0}$ & 2.15 & 0.89 & 3.42 & 1 & 5153 & 4596\\
\cellcolor{gray!6}{$\eta_{19, 0}$} & \cellcolor{gray!6}{1.53} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{2.27} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5437} & \cellcolor{gray!6}{4798}\\
$\eta_{20, 0}$ & 2.32 & 1.09 & 3.56 & 1 & 4709 & 3960\\
\cellcolor{gray!6}{$\eta_{21, 0}$} & \cellcolor{gray!6}{3.17} & \cellcolor{gray!6}{2.31} & \cellcolor{gray!6}{4.06} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4945} & \cellcolor{gray!6}{4942}\\
$\eta_{22, 0}$ & 1.80 & 0.71 & 2.91 & 1 & 4587 & 4935\\
\cellcolor{gray!6}{$\eta_{23, 0}$} & \cellcolor{gray!6}{2.23} & \cellcolor{gray!6}{0.90} & \cellcolor{gray!6}{3.52} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5388} & \cellcolor{gray!6}{5085}\\
$\eta_{24, 0}$ & 2.01 & 0.84 & 3.21 & 1 & 5657 & 5245\\
\cellcolor{gray!6}{$\eta_{25, 0}$} & \cellcolor{gray!6}{2.99} & \cellcolor{gray!6}{1.95} & \cellcolor{gray!6}{4.02} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5304} & \cellcolor{gray!6}{5342}\\
$\eta_{26, 0}$ & 1.23 & 0.23 & 2.22 & 1 & 5073 & 5183\\
\cellcolor{gray!6}{$\eta_{27, 0}$} & \cellcolor{gray!6}{1.41} & \cellcolor{gray!6}{0.56} & \cellcolor{gray!6}{2.29} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5099} & \cellcolor{gray!6}{4685}\\
$\eta_{28, 0}$ & 2.83 & 1.53 & 4.19 & 1 & 4565 & 4141\\
\cellcolor{gray!6}{$\eta_{29, 0}$} & \cellcolor{gray!6}{1.66} & \cellcolor{gray!6}{1.01} & \cellcolor{gray!6}{2.31} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5389} & \cellcolor{gray!6}{5000}\\
$\eta_{30, 0}$ & 1.06 & -0.11 & 2.21 & 1 & 5223 & 4882\\
\cellcolor{gray!6}{$\eta_{31, 0}$} & \cellcolor{gray!6}{2.36} & \cellcolor{gray!6}{1.20} & \cellcolor{gray!6}{3.54} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4672} & \cellcolor{gray!6}{4623}\\
$\eta_{32, 0}$ & 1.50 & 0.45 & 2.53 & 1 & 5322 & 5505\\
\cellcolor{gray!6}{$\eta_{33, 0}$} & \cellcolor{gray!6}{3.91} & \cellcolor{gray!6}{2.62} & \cellcolor{gray!6}{5.17} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5463} & \cellcolor{gray!6}{3971}\\
$\eta_{34, 0}$ & 3.09 & 2.22 & 3.95 & 1 & 5276 & 5101\\
\cellcolor{gray!6}{$\eta_{35, 0}$} & \cellcolor{gray!6}{1.51} & \cellcolor{gray!6}{0.38} & \cellcolor{gray!6}{2.58} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5251} & \cellcolor{gray!6}{5798}\\
$\eta_{36, 0}$ & 0.94 & -0.09 & 1.99 & 1 & 5452 & 4695\\
\cellcolor{gray!6}{$\eta_{1, 1}$} & \cellcolor{gray!6}{0.42} & \cellcolor{gray!6}{-1.14} & \cellcolor{gray!6}{1.97} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5577} & \cellcolor{gray!6}{5072}\\
$\eta_{2, 1}$ & 0.43 & -1.72 & 2.58 & 1 & 3792 & 2876\\
\cellcolor{gray!6}{$\eta_{3, 1}$} & \cellcolor{gray!6}{2.14} & \cellcolor{gray!6}{0.45} & \cellcolor{gray!6}{3.86} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4344} & \cellcolor{gray!6}{3558}\\
$\eta_{4, 1}$ & -0.05 & -1.86 & 1.76 & 1 & 5117 & 4595\\
\cellcolor{gray!6}{$\eta_{5, 1}$} & \cellcolor{gray!6}{-0.73} & \cellcolor{gray!6}{-2.73} & \cellcolor{gray!6}{1.16} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5122} & \cellcolor{gray!6}{4199}\\
$\eta_{6, 1}$ & 0.53 & -0.88 & 2.00 & 1 & 4175 & 3655\\
\cellcolor{gray!6}{$\eta_{7, 1}$} & \cellcolor{gray!6}{2.52} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{5.34} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4624} & \cellcolor{gray!6}{2815}\\
$\eta_{8, 1}$ & 0.13 & -1.47 & 1.63 & 1 & 4645 & 4650\\
\cellcolor{gray!6}{$\eta_{9, 1}$} & \cellcolor{gray!6}{-0.64} & \cellcolor{gray!6}{-3.48} & \cellcolor{gray!6}{1.85} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{3792} & \cellcolor{gray!6}{2442}\\
$\eta_{10, 1}$ & -0.33 & -1.73 & 1.05 & 1 & 4445 & 2443\\
\cellcolor{gray!6}{$\eta_{11, 1}$} & \cellcolor{gray!6}{-0.91} & \cellcolor{gray!6}{-2.31} & \cellcolor{gray!6}{0.45} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4892} & \cellcolor{gray!6}{3696}\\
$\eta_{12, 1}$ & -2.07 & -3.77 & -0.34 & 1 & 5612 & 5168\\
\cellcolor{gray!6}{$\eta_{13, 1}$} & \cellcolor{gray!6}{1.14} & \cellcolor{gray!6}{-0.28} & \cellcolor{gray!6}{2.66} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4393} & \cellcolor{gray!6}{3144}\\
$\eta_{14, 1}$ & -0.70 & -2.30 & 0.83 & 1 & 5105 & 4188\\
\cellcolor{gray!6}{$\eta_{15, 1}$} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{-2.20} & \cellcolor{gray!6}{2.41} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4181} & \cellcolor{gray!6}{2819}\\
$\eta_{16, 1}$ & 0.38 & -1.57 & 2.32 & 1 & 5455 & 3929\\
\cellcolor{gray!6}{$\eta_{17, 1}$} & \cellcolor{gray!6}{1.25} & \cellcolor{gray!6}{-0.42} & \cellcolor{gray!6}{2.97} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4592} & \cellcolor{gray!6}{4690}\\
$\eta_{18, 1}$ & 0.56 & -1.63 & 2.68 & 1 & 4374 & 3918\\
\cellcolor{gray!6}{$\eta_{19, 1}$} & \cellcolor{gray!6}{1.76} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{3.38} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5200} & \cellcolor{gray!6}{4890}\\
$\eta_{20, 1}$ & 3.89 & 1.64 & 6.23 & 1 & 5244 & 3261\\
\cellcolor{gray!6}{$\eta_{21, 1}$} & \cellcolor{gray!6}{-0.31} & \cellcolor{gray!6}{-2.45} & \cellcolor{gray!6}{1.68} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{3894} & \cellcolor{gray!6}{2628}\\
$\eta_{22, 1}$ & 1.23 & -0.57 & 3.01 & 1 & 4792 & 4052\\
\cellcolor{gray!6}{$\eta_{23, 1}$} & \cellcolor{gray!6}{1.42} & \cellcolor{gray!6}{-0.50} & \cellcolor{gray!6}{3.44} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5266} & \cellcolor{gray!6}{3701}\\
$\eta_{24, 1}$ & 0.32 & -1.33 & 1.91 & 1 & 4878 & 5305\\
\cellcolor{gray!6}{$\eta_{25, 1}$} & \cellcolor{gray!6}{1.68} & \cellcolor{gray!6}{-0.30} & \cellcolor{gray!6}{3.80} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4541} & \cellcolor{gray!6}{4510}\\
$\eta_{26, 1}$ & 1.00 & -0.54 & 2.56 & 1 & 5117 & 5050\\
\cellcolor{gray!6}{$\eta_{27, 1}$} & \cellcolor{gray!6}{0.94} & \cellcolor{gray!6}{-0.51} & \cellcolor{gray!6}{2.42} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4888} & \cellcolor{gray!6}{2971}\\
$\eta_{28, 1}$ & 2.87 & 0.93 & 4.89 & 1 & 4651 & 3564\\
\cellcolor{gray!6}{$\eta_{29, 1}$} & \cellcolor{gray!6}{-0.52} & \cellcolor{gray!6}{-1.81} & \cellcolor{gray!6}{0.72} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4373} & \cellcolor{gray!6}{3431}\\
$\eta_{30, 1}$ & 0.05 & -1.52 & 1.62 & 1 & 4931 & 4770\\
\cellcolor{gray!6}{$\eta_{31, 1}$} & \cellcolor{gray!6}{1.11} & \cellcolor{gray!6}{-1.27} & \cellcolor{gray!6}{3.49} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{3705} & \cellcolor{gray!6}{2305}\\
$\eta_{32, 1}$ & -0.22 & -1.77 & 1.31 & 1 & 5725 & 5907\\
\cellcolor{gray!6}{$\eta_{33, 1}$} & \cellcolor{gray!6}{2.85} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{6.08} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5826} & \cellcolor{gray!6}{4131}\\
$\eta_{34, 1}$ & 1.42 & -1.21 & 4.30 & 1 & 4895 & 4658\\
\cellcolor{gray!6}{$\eta_{35, 1}$} & \cellcolor{gray!6}{0.76} & \cellcolor{gray!6}{-0.87} & \cellcolor{gray!6}{2.45} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5231} & \cellcolor{gray!6}{5375}\\
$\eta_{36, 1}$ & -0.36 & -1.91 & 1.16 & 1 & 5127 & 6272\\*
\end{longtable}

==> tex-input/surv-example/0092-stage-two-psi-2-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{\label{tab:surv-stage-two-diag-psi-2}Stage two numeric diagnostics for $\psi_{2}$ in the survival example}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Stage two numeric diagnostics for $\psi_{2}$ in the survival example \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\theta_{0}$} & \cellcolor{gray!6}{-0.45} & \cellcolor{gray!6}{-1.65} & \cellcolor{gray!6}{0.69} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4554} & \cellcolor{gray!6}{8889}\\
$\theta_{1}$ & 0.26 & -0.07 & 0.61 & 1 & 9295 & 15161\\
\cellcolor{gray!6}{$\gamma$} & \cellcolor{gray!6}{7.23} & \cellcolor{gray!6}{4.02} & \cellcolor{gray!6}{10.58} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{11294} & \cellcolor{gray!6}{17823}\\
$\alpha$ & -0.51 & -1.17 & 0.05 & 1 & 3823 & 7811\\*
\end{longtable}

==> tex-input/surv-example/0100-point-est-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{Numerical diagnostics for the posterior of $\psi_{2}$ obtained using point estimates for both $\phi_{1 \cap 2}$ and $\phi_{2 \cap 3}$ in the survival example.}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Numerical diagnostics for the posterior of $\psi_{2}$ obtained using point estimates for both $\phi_{1 \cap 2}$ and $\phi_{2 \cap 3}$ in the survival example. \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\theta_{0}$} & \cellcolor{gray!6}{-0.10} & \cellcolor{gray!6}{-0.87} & \cellcolor{gray!6}{0.61} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12857} & \cellcolor{gray!6}{12870}\\
$\theta_{1}$ & 0.33 & 0.13 & 0.54 & 1 & 14232 & 14843\\
\cellcolor{gray!6}{$\gamma$} & \cellcolor{gray!6}{11.95} & \cellcolor{gray!6}{10.31} & \cellcolor{gray!6}{13.61} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{16361} & \cellcolor{gray!6}{12862}\\
$\alpha$ & -0.31 & -0.59 & -0.03 & 1 & 11984 & 13097\\*
\end{longtable}

==> tex-input/surv-example/0101-point-est-1-meld-23-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{Numerical diagnostics for the posterior of $\psi_{2}$ obtained using the point estimate for $\phi_{1 \cap 2}$ in the survival example.}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Numerical diagnostics for the posterior of $\psi_{2}$ obtained using the point estimate for $\phi_{1 \cap 2}$ in the survival example. \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\theta_{0}$} & \cellcolor{gray!6}{-0.06} & \cellcolor{gray!6}{-0.84} & \cellcolor{gray!6}{0.70} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{7253} & \cellcolor{gray!6}{8306}\\
$\theta_{1}$ & 0.34 & 0.14 & 0.56 & 1 & 14190 & 18763\\
\cellcolor{gray!6}{$\gamma$} & \cellcolor{gray!6}{11.97} & \cellcolor{gray!6}{10.37} & \cellcolor{gray!6}{13.58} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24246} & \cellcolor{gray!6}{21608}\\
$\alpha$ & -0.33 & -0.66 & -0.04 & 1 & 6333 & 8391\\*
\end{longtable}

==> tex-input/surv-example/0102-point-est-3-meld-12-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{Numerical diagnostics for the posterior of $\psi_{2}$ obtained using the point estimate for $\phi_{2 \cap 3}$ in the survival example.}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Numerical diagnostics for the posterior of $\psi_{2}$ obtained using the point estimate for $\phi_{2 \cap 3}$ in the survival example. \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\theta_{0}$} & \cellcolor{gray!6}{-0.53} & \cellcolor{gray!6}{-1.71} & \cellcolor{gray!6}{0.62} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{6868} & \cellcolor{gray!6}{10365}\\
$\theta_{1}$ & 0.25 & -0.08 & 0.59 & 1 & 13405 & 19867\\
\cellcolor{gray!6}{$\gamma$} & \cellcolor{gray!6}{7.11} & \cellcolor{gray!6}{3.84} & \cellcolor{gray!6}{10.52} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{11474} & \cellcolor{gray!6}{17440}\\
$\alpha$ & -0.46 & -1.06 & 0.07 & 1 & 5960 & 10535\\*
\end{longtable}

==> tex-input/surv-example/0103-point-est-3-meld-12-phi-12-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{Numerical diagnostics for $\phi_{1 \cap 2}$ when $\phi_{2 \cap 3}$ is fixed and submodels $\pd_{1}$ and $\pd_{2}$ are melded.}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Numerical diagnostics for $\phi_{1 \cap 2}$ when $\phi_{2 \cap 3}$ is fixed and submodels $\pd_{1}$ and $\pd_{2}$ are melded. \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$T_{1}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25014} & \cellcolor{gray!6}{24995}\\
$T_{2}$ & 0.97 & 0.83 & 1.00 & 1 & 13102 & 24995\\
\cellcolor{gray!6}{$T_{3}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.90} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{11334} & \cellcolor{gray!6}{24995}\\
$T_{4}$ & 1.00 & 1.00 & 1.00 & 1 & 25018 & 24995\\
\cellcolor{gray!6}{$T_{5}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$T_{6}$ & 0.91 & 0.75 & 1.00 & 1 & 6681 & 24995\\
\cellcolor{gray!6}{$T_{7}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.98} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{16729} & \cellcolor{gray!6}{24995}\\
$T_{8}$ & 1.00 & 1.00 & 1.00 & 1 & 22845 & 24995\\
\cellcolor{gray!6}{$T_{9}$} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{0.56} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{2485} & \cellcolor{gray!6}{24995}\\
$T_{10}$ & 0.80 & 0.69 & 0.94 & 1 & 6062 & 3081\\
\cellcolor{gray!6}{$T_{11}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.91} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{19751} & \cellcolor{gray!6}{24995}\\
$T_{12}$ & 0.95 & 0.82 & 1.00 & 1 & 11912 & 24995\\
\cellcolor{gray!6}{$T_{13}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22245} & \cellcolor{gray!6}{24995}\\
$T_{14}$ & 1.00 & 1.00 & 1.00 & 1 & 25010 & 24995\\
\cellcolor{gray!6}{$T_{15}$} & \cellcolor{gray!6}{0.96} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{11245} & \cellcolor{gray!6}{24995}\\
$T_{16}$ & 1.00 & 1.00 & 1.00 & 1 & 24112 & 24995\\
\cellcolor{gray!6}{$T_{17}$} & \cellcolor{gray!6}{0.98} & \cellcolor{gray!6}{0.88} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12999} & \cellcolor{gray!6}{24995}\\
$T_{18}$ & 0.94 & 0.74 & 1.00 & 1 & 7165 & 24995\\
\cellcolor{gray!6}{$T_{19}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$T_{20}$ & 0.98 & 0.85 & 1.00 & 1 & 6541 & 24995\\
\cellcolor{gray!6}{$T_{21}$} & \cellcolor{gray!6}{0.91} & \cellcolor{gray!6}{0.74} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{8703} & \cellcolor{gray!6}{24995}\\
$T_{22}$ & 0.92 & 0.72 & 1.00 & 1 & 5301 & 24995\\
\cellcolor{gray!6}{$T_{23}$} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{0.82} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{9463} & \cellcolor{gray!6}{24995}\\
$T_{24}$ & 1.00 & 1.00 & 1.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$T_{25}$} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{8008} & \cellcolor{gray!6}{24995}\\
$T_{26}$ & 1.00 & 1.00 & 1.00 & 1 & 25018 & 24995\\
\cellcolor{gray!6}{$T_{27}$} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{0.84} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12215} & \cellcolor{gray!6}{24995}\\
$T_{28}$ & 0.99 & 0.93 & 1.00 & 1 & 10717 & 24995\\
\cellcolor{gray!6}{$T_{29}$} & \cellcolor{gray!6}{0.99} & \cellcolor{gray!6}{0.94} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{21176} & \cellcolor{gray!6}{24995}\\
$T_{30}$ & 1.00 & 1.00 & 1.00 & 1 & 25010 & 24995\\
\cellcolor{gray!6}{$T_{31}$} & \cellcolor{gray!6}{0.88} & \cellcolor{gray!6}{0.65} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{3612} & \cellcolor{gray!6}{24995}\\
$T_{32}$ & 1.00 & 1.00 & 1.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$T_{33}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24099} & \cellcolor{gray!6}{24995}\\
$T_{34}$ & 0.99 & 0.93 & 1.00 & 1 & 16980 & 24995\\
\cellcolor{gray!6}{$T_{35}$} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$T_{36}$ & 1.00 & 1.00 & 1.00 & 1 & 22095 & 24995\\
\cellcolor{gray!6}{$\delta_{1}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{25014} & \cellcolor{gray!6}{25014}\\
$\delta_{2}$ & 0.33 & 0.00 & 1.00 & 1 & 12562 & 24995\\
\cellcolor{gray!6}{$\delta_{3}$} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{10970} & \cellcolor{gray!6}{24995}\\
$\delta_{4}$ & 0.00 & 0.00 & 0.00 & 1 & 25018 & 25018\\
\cellcolor{gray!6}{$\delta_{5}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$\delta_{6}$ & 0.70 & 0.00 & 1.00 & 1 & 4904 & 24995\\
\cellcolor{gray!6}{$\delta_{7}$} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{16319} & \cellcolor{gray!6}{24995}\\
$\delta_{8}$ & 0.02 & 0.00 & 0.00 & 1 & 22759 & 22759\\
\cellcolor{gray!6}{$\delta_{9}$} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{2007} & \cellcolor{gray!6}{24995}\\
$\delta_{10}$ & 0.99 & 1.00 & 1.00 & 1 & 2227 & 24995\\
\cellcolor{gray!6}{$\delta_{11}$} & \cellcolor{gray!6}{0.24} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{16504} & \cellcolor{gray!6}{24995}\\
$\delta_{12}$ & 0.62 & 0.00 & 1.00 & 1 & 10373 & 24995\\
\cellcolor{gray!6}{$\delta_{13}$} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{22208} & \cellcolor{gray!6}{22208}\\
$\delta_{14}$ & 0.00 & 0.00 & 0.00 & 1 & 25010 & 25010\\
\cellcolor{gray!6}{$\delta_{15}$} & \cellcolor{gray!6}{0.39} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{10706} & \cellcolor{gray!6}{24995}\\
$\delta_{16}$ & 0.00 & 0.00 & 0.00 & 1 & 24074 & 24074\\
\cellcolor{gray!6}{$\delta_{17}$} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{12081} & \cellcolor{gray!6}{24995}\\
$\delta_{18}$ & 0.46 & 0.00 & 1.00 & 1 & 6399 & 24995\\
\cellcolor{gray!6}{$\delta_{19}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$\delta_{20}$ & 0.16 & 0.00 & 1.00 & 1 & 6136 & 24995\\
\cellcolor{gray!6}{$\delta_{21}$} & \cellcolor{gray!6}{0.71} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{7401} & \cellcolor{gray!6}{24995}\\
$\delta_{22}$ & 0.54 & 0.00 & 1.00 & 1 & 4496 & 24995\\
\cellcolor{gray!6}{$\delta_{23}$} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{9020} & \cellcolor{gray!6}{24995}\\
$\delta_{24}$ & 0.00 & 0.00 & 0.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$\delta_{25}$} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{7418} & \cellcolor{gray!6}{24995}\\
$\delta_{26}$ & 0.00 & 0.00 & 0.00 & 1 & 25018 & 25018\\
\cellcolor{gray!6}{$\delta_{27}$} & \cellcolor{gray!6}{0.28} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{11493} & \cellcolor{gray!6}{24995}\\
$\delta_{28}$ & 0.08 & 0.00 & 1.00 & 1 & 10508 & 24995\\
\cellcolor{gray!6}{$\delta_{29}$} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{19988} & \cellcolor{gray!6}{24995}\\
$\delta_{30}$ & 0.00 & 0.00 & 0.00 & 1 & 25010 & 25010\\
\cellcolor{gray!6}{$\delta_{31}$} & \cellcolor{gray!6}{0.67} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{2738} & \cellcolor{gray!6}{24995}\\
$\delta_{32}$ & 0.00 & 0.00 & 0.00 & 1 & 24995 & 24995\\
\cellcolor{gray!6}{$\delta_{33}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24157} & \cellcolor{gray!6}{24157}\\
$\delta_{34}$ & 0.09 & 0.00 & 1.00 & 1 & 16700 & 24995\\
\cellcolor{gray!6}{$\delta_{35}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{24995} & \cellcolor{gray!6}{24995}\\
$\delta_{36}$ & 0.03 & 0.00 & 0.00 & 1 & 21567 & 21567\\*
\end{longtable}

==> tex-input/surv-example/0104-point-est-1-meld-23-phi-23-diag.tex <==

\begin{longtable}[t]{lrrrrrr}
\caption{Numerical diagnostics for $\phi_{2 \cap 3}$ when $\phi_{1 \cap 2}$ is fixed and submodels $\pd_{2}$ and $\pd_{3}$ are melded.}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endfirsthead
\caption[]{Numerical diagnostics for $\phi_{2 \cap 3}$ when $\phi_{1 \cap 2}$ is fixed and submodels $\pd_{2}$ and $\pd_{3}$ are melded. \textit{(continued)}}\\
\toprule
  & Mean & $q_{0.05}$ & $q_{0.95}$ & $\widehat{R}$ & $\widehat{\text{ESS}}_{B}$ & $\widehat{\text{ESS}}_{T}$\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
\cellcolor{gray!6}{$\eta_{0, 1}$} & \cellcolor{gray!6}{0.59} & \cellcolor{gray!6}{-0.24} & \cellcolor{gray!6}{1.43} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5242} & \cellcolor{gray!6}{5634}\\
$\eta_{0, 2}$ & 1.52 & 0.37 & 2.64 & 1 & 5460 & 5251\\
\cellcolor{gray!6}{$\eta_{0, 3}$} & \cellcolor{gray!6}{3.22} & \cellcolor{gray!6}{2.21} & \cellcolor{gray!6}{4.21} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5404} & \cellcolor{gray!6}{5461}\\
$\eta_{0, 4}$ & 1.98 & 0.68 & 3.30 & 1 & 6276 & 4990\\
\cellcolor{gray!6}{$\eta_{0, 5}$} & \cellcolor{gray!6}{1.23} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{2.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5802} & \cellcolor{gray!6}{5603}\\
$\eta_{0, 6}$ & 1.04 & 0.27 & 1.84 & 1 & 5204 & 5143\\
\cellcolor{gray!6}{$\eta_{0, 7}$} & \cellcolor{gray!6}{4.04} & \cellcolor{gray!6}{2.65} & \cellcolor{gray!6}{5.41} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{6373} & \cellcolor{gray!6}{5634}\\
$\eta_{0, 8}$ & 1.74 & 0.67 & 2.80 & 1 & 4657 & 2781\\
\cellcolor{gray!6}{$\eta_{0, 9}$} & \cellcolor{gray!6}{1.12} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{2.02} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5281} & \cellcolor{gray!6}{5729}\\
$\eta_{0, 10}$ & 1.36 & 0.72 & 2.01 & 1 & 5967 & 5779\\
\cellcolor{gray!6}{$\eta_{0, 11}$} & \cellcolor{gray!6}{2.21} & \cellcolor{gray!6}{1.45} & \cellcolor{gray!6}{3.00} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{6115} & \cellcolor{gray!6}{5744}\\
$\eta_{0, 12}$ & 2.53 & 1.54 & 3.55 & 1 & 5677 & 5308\\
\cellcolor{gray!6}{$\eta_{0, 13}$} & \cellcolor{gray!6}{2.22} & \cellcolor{gray!6}{1.29} & \cellcolor{gray!6}{3.15} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5564} & \cellcolor{gray!6}{4966}\\
$\eta_{0, 14}$ & 1.25 & 0.19 & 2.31 & 1 & 5249 & 5352\\
\cellcolor{gray!6}{$\eta_{0, 15}$} & \cellcolor{gray!6}{1.15} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{2.06} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{6167} & \cellcolor{gray!6}{5103}\\
$\eta_{0, 16}$ & 1.01 & -0.14 & 2.18 & 1 & 6876 & 6588\\
\cellcolor{gray!6}{$\eta_{0, 17}$} & \cellcolor{gray!6}{1.64} & \cellcolor{gray!6}{0.80} & \cellcolor{gray!6}{2.50} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{6554} & \cellcolor{gray!6}{6604}\\
$\eta_{0, 18}$ & 2.17 & 0.94 & 3.50 & 1 & 4214 & 2032\\
\cellcolor{gray!6}{$\eta_{0, 19}$} & \cellcolor{gray!6}{1.52} & \cellcolor{gray!6}{0.75} & \cellcolor{gray!6}{2.30} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5041} & \cellcolor{gray!6}{4290}\\
$\eta_{0, 20}$ & 2.34 & 1.15 & 3.57 & 1 & 6437 & 6173\\
\cellcolor{gray!6}{$\eta_{0, 21}$} & \cellcolor{gray!6}{3.15} & \cellcolor{gray!6}{2.30} & \cellcolor{gray!6}{4.02} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4752} & \cellcolor{gray!6}{2725}\\
$\eta_{0, 22}$ & 1.81 & 0.73 & 2.91 & 1 & 4376 & 2835\\
\cellcolor{gray!6}{$\eta_{0, 23}$} & \cellcolor{gray!6}{2.25} & \cellcolor{gray!6}{0.91} & \cellcolor{gray!6}{3.53} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5348} & \cellcolor{gray!6}{5857}\\
$\eta_{0, 24}$ & 2.00 & 0.83 & 3.20 & 1 & 5817 & 5773\\
\cellcolor{gray!6}{$\eta_{0, 25}$} & \cellcolor{gray!6}{2.99} & \cellcolor{gray!6}{2.01} & \cellcolor{gray!6}{3.99} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5715} & \cellcolor{gray!6}{5483}\\
$\eta_{0, 26}$ & 1.23 & 0.28 & 2.23 & 1 & 5432 & 5123\\
\cellcolor{gray!6}{$\eta_{0, 27}$} & \cellcolor{gray!6}{1.39} & \cellcolor{gray!6}{0.56} & \cellcolor{gray!6}{2.27} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5165} & \cellcolor{gray!6}{4639}\\
$\eta_{0, 28}$ & 2.86 & 1.56 & 4.23 & 1 & 5163 & 3967\\
\cellcolor{gray!6}{$\eta_{0, 29}$} & \cellcolor{gray!6}{1.65} & \cellcolor{gray!6}{1.01} & \cellcolor{gray!6}{2.29} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5895} & \cellcolor{gray!6}{4268}\\
$\eta_{0, 30}$ & 1.08 & -0.06 & 2.21 & 1 & 5858 & 5995\\
\cellcolor{gray!6}{$\eta_{0, 31}$} & \cellcolor{gray!6}{2.32} & \cellcolor{gray!6}{1.17} & \cellcolor{gray!6}{3.46} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4239} & \cellcolor{gray!6}{2892}\\
$\eta_{0, 32}$ & 1.48 & 0.43 & 2.52 & 1 & 5707 & 5442\\
\cellcolor{gray!6}{$\eta_{0, 33}$} & \cellcolor{gray!6}{3.94} & \cellcolor{gray!6}{2.67} & \cellcolor{gray!6}{5.19} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4882} & \cellcolor{gray!6}{2769}\\
$\eta_{0, 34}$ & 3.08 & 2.21 & 3.97 & 1 & 5751 & 4254\\
\cellcolor{gray!6}{$\eta_{0, 35}$} & \cellcolor{gray!6}{1.52} & \cellcolor{gray!6}{0.38} & \cellcolor{gray!6}{2.61} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5114} & \cellcolor{gray!6}{2660}\\
$\eta_{0, 36}$ & 0.92 & -0.11 & 1.93 & 1 & 6337 & 6140\\
\cellcolor{gray!6}{$\eta_{1, 1}$} & \cellcolor{gray!6}{0.44} & \cellcolor{gray!6}{-1.11} & \cellcolor{gray!6}{1.97} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4600} & \cellcolor{gray!6}{5035}\\
$\eta_{1, 2}$ & 0.32 & -1.79 & 2.34 & 1 & 6096 & 4726\\
\cellcolor{gray!6}{$\eta_{1, 3}$} & \cellcolor{gray!6}{2.17} & \cellcolor{gray!6}{0.43} & \cellcolor{gray!6}{3.94} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5630} & \cellcolor{gray!6}{4928}\\
$\eta_{1, 4}$ & 0.01 & -1.73 & 1.73 & 1 & 6487 & 6133\\
\cellcolor{gray!6}{$\eta_{1, 5}$} & \cellcolor{gray!6}{-0.72} & \cellcolor{gray!6}{-2.64} & \cellcolor{gray!6}{1.11} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5809} & \cellcolor{gray!6}{3579}\\
$\eta_{1, 6}$ & 0.53 & -0.82 & 1.93 & 1 & 5921 & 5189\\
\cellcolor{gray!6}{$\eta_{1, 7}$} & \cellcolor{gray!6}{2.54} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{5.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5798} & \cellcolor{gray!6}{6369}\\
$\eta_{1, 8}$ & 0.17 & -1.43 & 1.73 & 1 & 5051 & 3228\\
\cellcolor{gray!6}{$\eta_{1, 9}$} & \cellcolor{gray!6}{-0.46} & \cellcolor{gray!6}{-3.14} & \cellcolor{gray!6}{1.94} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5276} & \cellcolor{gray!6}{4483}\\
$\eta_{1, 10}$ & -0.31 & -1.69 & 1.06 & 1 & 5312 & 4881\\
\cellcolor{gray!6}{$\eta_{1, 11}$} & \cellcolor{gray!6}{-0.83} & \cellcolor{gray!6}{-2.18} & \cellcolor{gray!6}{0.53} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5170} & \cellcolor{gray!6}{2888}\\
$\eta_{1, 12}$ & -1.93 & -3.68 & -0.26 & 1 & 5456 & 4877\\
\cellcolor{gray!6}{$\eta_{1, 13}$} & \cellcolor{gray!6}{1.17} & \cellcolor{gray!6}{-0.25} & \cellcolor{gray!6}{2.65} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5876} & \cellcolor{gray!6}{4898}\\
$\eta_{1, 14}$ & -0.70 & -2.29 & 0.85 & 1 & 5292 & 3918\\
\cellcolor{gray!6}{$\eta_{1, 15}$} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{-2.24} & \cellcolor{gray!6}{2.17} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{6210} & \cellcolor{gray!6}{4838}\\
$\eta_{1, 16}$ & 0.41 & -1.50 & 2.29 & 1 & 5985 & 4945\\
\cellcolor{gray!6}{$\eta_{1, 17}$} & \cellcolor{gray!6}{1.32} & \cellcolor{gray!6}{-0.32} & \cellcolor{gray!6}{2.99} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5967} & \cellcolor{gray!6}{5379}\\
$\eta_{1, 18}$ & 0.38 & -1.85 & 2.48 & 1 & 4067 & 1276\\
\cellcolor{gray!6}{$\eta_{1, 19}$} & \cellcolor{gray!6}{1.76} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{3.44} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5302} & \cellcolor{gray!6}{5240}\\
$\eta_{1, 20}$ & 3.63 & 1.36 & 5.96 & 1 & 5309 & 4271\\
\cellcolor{gray!6}{$\eta_{1, 21}$} & \cellcolor{gray!6}{-0.30} & \cellcolor{gray!6}{-2.40} & \cellcolor{gray!6}{1.65} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4736} & \cellcolor{gray!6}{1994}\\
$\eta_{1, 22}$ & 1.13 & -0.62 & 2.93 & 1 & 4450 & 2348\\
\cellcolor{gray!6}{$\eta_{1, 23}$} & \cellcolor{gray!6}{1.29} & \cellcolor{gray!6}{-0.59} & \cellcolor{gray!6}{3.27} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5678} & \cellcolor{gray!6}{5057}\\
$\eta_{1, 24}$ & 0.37 & -1.22 & 2.00 & 1 & 4709 & 2427\\
\cellcolor{gray!6}{$\eta_{1, 25}$} & \cellcolor{gray!6}{1.53} & \cellcolor{gray!6}{-0.38} & \cellcolor{gray!6}{3.55} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5926} & \cellcolor{gray!6}{3849}\\
$\eta_{1, 26}$ & 0.99 & -0.53 & 2.54 & 1 & 3684 & 2816\\
\cellcolor{gray!6}{$\eta_{1, 27}$} & \cellcolor{gray!6}{0.89} & \cellcolor{gray!6}{-0.52} & \cellcolor{gray!6}{2.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5718} & \cellcolor{gray!6}{5561}\\
$\eta_{1, 28}$ & 2.86 & 0.90 & 4.82 & 1 & 5379 & 3891\\
\cellcolor{gray!6}{$\eta_{1, 29}$} & \cellcolor{gray!6}{-0.48} & \cellcolor{gray!6}{-1.75} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{6388} & \cellcolor{gray!6}{6400}\\
$\eta_{1, 30}$ & 0.05 & -1.49 & 1.62 & 1 & 6180 & 3753\\
\cellcolor{gray!6}{$\eta_{1, 31}$} & \cellcolor{gray!6}{1.09} & \cellcolor{gray!6}{-1.12} & \cellcolor{gray!6}{3.36} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{4454} & \cellcolor{gray!6}{2390}\\
$\eta_{1, 32}$ & -0.19 & -1.80 & 1.36 & 1 & 5709 & 5724\\
\cellcolor{gray!6}{$\eta_{1, 33}$} & \cellcolor{gray!6}{2.85} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{6.11} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5190} & \cellcolor{gray!6}{5496}\\
$\eta_{1, 34}$ & 1.51 & -0.99 & 4.29 & 1 & 5964 & 6177\\
\cellcolor{gray!6}{$\eta_{1, 35}$} & \cellcolor{gray!6}{0.73} & \cellcolor{gray!6}{-0.88} & \cellcolor{gray!6}{2.49} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{5041} & \cellcolor{gray!6}{2357}\\
$\eta_{1, 36}$ & -0.33 & -1.91 & 1.16 & 1 & 6111 & 6548\\*
\end{longtable}
